Fully kinetic model of plasma expansion in a magnetic nozzle

A self-consistent model is presented for performing steady-state fully kinetic Particle-in-Cell simulations of magnetised plasma plumes. An energy-based electron reflection prevents the numerical pump instability associated with a typical open-outflow boundary, and is shown to be sufficiently general that both the plume kinetics and plasma potential demonstrate domain independence (within 4%). This is upheld by non-stationary Robin-type boundary conditions on the Poisson's equation, coupled to a capacitive circuit that allows physical evolution of the downstream potential drop in the transient. The method has been validated against experiments, providing results that fall within the uncertainty of measurements. Simulations are then carried out to study collisional xenon discharges into axisymmetric diverging magnetic nozzles. Particular discussion is given to the identification of a potential well arising from charge separation at the edge of the plume, the role of ion-neutral charge exchange, and a three-region piecewise polytropic cooling regime for electrons. The polytropic index is shown to depend on the degree of magnetisation. Specifically, in the region near the thruster outlet, the plume is weakly-magnetised due to the cross-field diffusion of electron-heavy particle collisions. Downstream, a strongly-magnetised region of near-isothermal expansion occurs. Finally, in the detached region, the polytropic index tends to that of a more adiabatic unmagnetised case. With an increasing magnetic nozzle field strength, an inferior limit is found to the average polytropic index of $\bar{\gamma}_e\sim1.16$.

==> chap_1_MM.tex <==
\section{Introduction}

The study of electric propulsion continues to receive much attention despite mature technologies such as Ion and Hall effect thruster establishing dominant flight heritage over the last two decades. However, such systems are increasingly being recognised as complex and high cost, particularly for small-satellite propulsion \cite{b:keidar2014}. Therefore, in the last few years, particular effort has been put into the development of magnetically-enhanced plasma thrusters (MEPT). {\color{red} This broad category includes the Helicon Plasma Thruster (HPT) \cite{b:pavarin2010,b:boswell2003,b:shinohara2014,b:merino2015}, the Electron Cyclotron Resonance Thruster (ECRT) \cite{b:cannat2015}, and the Applied Field MagnetoPlasma Dynamic Thruster (AF-MPDT) \cite{b:boxberger2019}. In such systems the acceleration of the plasma is driven by a magnetic nozzle (MN) \cite{b:merino2016}: a divergent magneto-static field generated by a set of solenoids or permanent magnets.} {\color{blue}The MN radially confines the hot partially-magnetised plasma beam and accelerates it supersonically via the conversion of thermal energy into directed axial kinetic energy \cite{b:magarotto2020}, therefore enhancing thrust.}

The HPT and ECRT are cathode-less devices, relying on electromagnetic waves for plasma production and heating, while the AF-MPDT relies on annular electrodes. Since the resulting plasma beam is quasi-neutral, no additional neutraliser (e.g. a hollow cathode) is required. Thus, MEPTs are becoming an increasing option for low-thrust propulsion, being highly scalable, robust, light, low-cost and resistant to lifetime-limiting erosion \cite{b:manente2018}. MNs have no walls, thus avoiding thermal loading and erosion issues. The first in-orbit demonstration of a radiofrequency MEPT took place from March 2021 by Technology for Innovation and Propulsion (T4i) S.p.A. with the 50W ‘‘REGULUS’’ thruster  \cite{b:bellomo2019,b:bellomo2021}. At the same time, the present disadvantage of MEPTs is the relatively low thrust efficiency, generally $<$20\% \cite{b:takahashi2019}. For MEPTs to be sufficiently efficient and competitive, a high ionisation ratio is mandatory (with electron temperatures of tens of eV \cite{b:magarotto2020_2}) or else the specific impulse achievable with the MN is limited.

{\color{red} The main MN physics is reasonably established and understood. In typical MEPTs, with magnetic fields in the 100-1000G range, ions are weakly magnetised and are bound to the highly magnetised electrons through an ambipolar electric field, which develops to maintain quasi-neutrality \cite{b:longmier2011,b:olsen2015}.} {\color{blue}This results in a potential drop, both radially and axially, which confines most of the electron population while accelerating ions freely downstream. The potential drop along the MN self-consistently evolves to maintain a globally current-free plasma, ultimately determining the velocity of ions \cite{b:lafleur2015}}. Nonetheless, there are many other aspects requiring further detailed investigation, such as the evolution of velocity distribution functions, plasma detachment, anisotropic electron cooling and doubly-trapped electron populations \cite{b:kaganovich2020}.

Numerical efforts to understand MNs have involved both fluid and kinetic models, some of which make use of semi-analytical solutions \cite{b:merino2018kinetic,b:sasoh1994}. Two-dimensional (2D) fluid models have shown to be a powerful tool to understand the main phenomena in the MN \cite{b:ahedo2010}. {\color{blue}However, their closure (i.e. a definition of non-local heat conduction) remains an elusive problem.} One-dimensional (1D) stationary kinetic models of a MN have allowed analysing the downstream ion and electron heat fluxes and the response to non-Maxwellian features of the ion and electron velocity distribution functions (VDF) \cite{b:martinez2015,b:ahedo2020}. However, except for 1D cases, solving the Boltzmann equation directly is often computationally intensive \cite{b:kim2005}. {\color{red}Both fluid and kinetic continuum approaches must also make assumptions regarding the VDF, one of the main impact parameters in magnetised plasma expansion \cite{b:ahedo2020}. Therefore, numerical studies need to be extended to fully-kinetic \cite{b:difede2021,b:porto2019} or fluid/kinetic \cite{b:alvaro2021} approaches if the dynamics of a MN want to be treated self-consistently.} The fully-kinetic Particle-in-Cell (PIC) method represents the numerical strategy with the lowest level of assumptions. Both electron and ion populations are modelled as macro-particles, subject to the action of {\color{red}self-consistently computed} electric and magnetic fields, as well as particle collisions \cite{b:birdsall1991}.

{\color{red}PIC simulations operate by necessity on a finite domain. Nonetheless a potential drop occurs along the MN concurrently to the ambipolar electric field. For a typical meso-thermal plume (electron thermal velocity greatly exceeds the ion drift velocity and ion thermal velocity), most of the electron population is trapped by this potential drop. Namely, electron trajectories reverse before particles escape to the infinity \cite{b:merino2019iepc,b:li2019}. Since the computational domain is finite, the location of this reversal may exist beyond the domain. As a result, the definition of consistent downstream (and lateral) boundary conditions is a challenging and not fully solved problem. For instance, if electrons are non-physically deleted when reaching the external open boundary, the so called ‘‘numerical pump instability’’ can arise \cite{b:briedaThesis,b:brieda2018}.} For this reason simulations are usually stopped long before the ion beam reaches the outer boundaries. {\color{red}Thus, most results in the literature deal with transient plume expansions in small domains \cite{b:levin2018, b:hu2017}. Alternatively, a virtual ion sink was implemented midway between the inlet and outlet boundaries \cite{b:brieda2018}. Ions are absorbed by the sink while electrons can permeate through it, thus retaining the trapped electrons between the ion sink and the boundary. However, the sink must be located far from the computational boundary, resulting in an increase in the domain size. In order to overcome this limitation, a charge-conserving boundary condition has been proposed \cite{b:levin2020} where the number of electrons reflected at the open boundary is determined to maintain the plasma globally-neutral. Another approach formulated to mimic the real physics involves a current-free boundary condition \cite{b:li2019}. The latter has been demonstrated via simulations of both a non-magnetized plume \cite{b:li2019} and a MN \cite{b:chen2020}. The methodology proposed in these works \cite{b:li2019,b:chen2020} is convincing for what the particles motion is concerned, but simplified conditions have been assumed for the solution of the electromagnetic fields. A zero gradient Neumann condition has been imposed at the open boundary to solve the Poisson's equation.} Such a condition is appropriate only in the limit of an infinitely large domain that encompasses nearly all the potential fall that occurs in the plasma plume. For this reason, the authors of \cite{b:li2019} suggest to ignore the plasma dynamics in some portion of the domain near the outer boundaries (i.e., $\approx$20\%). 

{\color{red}This article presents a new methodology to study the plasma expansions in a MN by means of an electrostatic PIC code. Boundary conditions are defined to improve on previous works in terms of electron kinetics and Poisson equation. Regarding the treatment of the electrons, a consistent approach has been defined to selectively reflect or absorb part of the particles crossing the boundaries. An integral current-free condition along the outer edge of the domain and an energy-based reflection criterion on electrons have been enforced. The total potential drop is self-consistently calculated to maintain the current-free condition. Its value is adopted to define a Robin boundary condition on the plasma potential. As a result, a set of mutually consistent boundary conditions has been defined which is sufficiently general to provide results almost independent of the computational domain size and in good agreement with experiments \cite{b:lafleur2011}.}

Section 2 summarises the key aspects of the PIC model and introduces the new boundary condition treatment. {\color{red}In Section 3 the capability to produce a stable steady-state plume and a solution which is not dependent on the domain size have been proven. In section 4 the numerical approach has been benchmarked against measures of plasma density and electrostatic potential \cite{b:lafleur2011}. In section 5 the validated approach has been exploited to investigate the plume expansion in a MN. The most relevant aspects analysed are: the presence of a radial potential well that affects the plasma dynamics, the influence that the intensity of the magnetic field has on the propulsive performance, and the evolution of the electron VDF.} The conclusions are then given in Section 6.

==> chap_1_SA.tex <==
\section{Introduction}

The study of electric propulsion continues to receive much attention despite mature technologies such as Ion and Hall effect thruster establishing dominant flight heritage over the last two decades. However, such systems are increasingly being recognised as complex and high cost, particularly for small-satellite {\color{blue}applications} \cite{b:keidar2014}. Therefore, in the last few years, particular effort has been made in the development of magnetically-enhanced plasma thrusters (MEPT). {\color{red} This broad category includes the Helicon Plasma Thruster (HPT) \cite{b:pavarin2010,b:boswell2003,b:shinohara2014,b:merino2015}, the Electron Cyclotron Resonance Thruster (ECRT) \cite{b:cannat2015}, and the Applied Field MagnetoPlasma Dynamic Thruster (AF-MPDT) \cite{b:boxberger2019}. In such systems the {\color{blue} plasma acceleration} is driven by a magnetic nozzle (MN) \cite{b:merino2016}: a divergent magneto-static field generated by a set of solenoids or permanent magnets.} {\color{blue}The MN radially confines the hot partially-magnetised plasma beam and accelerates it supersonically via the conversion of thermal energy into directed axial kinetic energy \cite{b:magarotto2020}, therefore enhancing thrust.}

The HPT and ECRT are cathode-less devices, relying on electromagnetic waves for plasma production and heating, while the AF-MPDT relies on annular electrodes. Since the resulting plasma beam is quasi-neutral, no additional neutraliser (e.g. a hollow cathode) is required. Thus, MEPTs are becoming an increasing option for low-thrust propulsion, being highly scalable, robust, light, low-cost and resistant to lifetime-limiting erosion \cite{b:manente2018}. MNs also have no physical walls, thus avoiding thermal loading and erosion issues. The first in-orbit demonstration of a radio-frequency MEPT took place from March 2021 by Technology for Innovation and Propulsion (T4i) S.p.A. with the 50W ‘‘REGULUS’’ thruster  \cite{b:bellomo2019,b:bellomo2021}. At the same time, the present disadvantage of MEPTs is the relatively low thrust efficiency, generally $<$20\% \cite{b:takahashi2019}. For MEPTs to be sufficiently efficient and competitive, a high ionisation ratio is mandatory (with electron temperatures of tens of eV \cite{b:magarotto2020_2}) or else the specific impulse achievable with the MN is limited.

{\color{red} The main MN physics is reasonably established and understood. In typical MEPTs, with magnetic fields in the 100-1000G range, ions are weakly magnetised and are bound to the highly magnetised electrons through an ambipolar electric field, which develops to maintain quasi-neutrality \cite{b:longmier2011,b:olsen2015}.} {\color{blue}This results in a potential drop, both radially and axially, which confines most of the electron population while accelerating ions freely downstream. The potential drop self-consistently evolves to maintain a globally current-free plasma, ultimately determining the velocity of ions \cite{b:lafleur2015}}. Nevertheless, there are many other aspects requiring further detailed investigation, such as the evolution of velocity distribution functions (VDF), plasma detachment, anisotropic electron cooling and doubly-trapped electron populations \cite{b:kaganovich2020}.

Numerical efforts to understand MNs have involved both fluid and kinetic models, some of which make use of semi-analytical solutions \cite{b:merino2018kinetic,b:sasoh1994}. Two-dimensional (2D) fluid models have shown to be a powerful tool to understand the main phenomena in the MN \cite{b:ahedo2010}. {\color{blue}However, their closure (i.e. a definition of non-local heat conduction) remains an elusive problem.} One-dimensional (1D) stationary kinetic models of a MN have allowed analysis of the downstream ion and electron heat fluxes and the response to non-Maxwellian features of the ion and electron VDFs \cite{b:martinez2015,b:ahedo2020}. However, except for 1D cases, solving the Boltzmann equation directly is often computationally intensive \cite{b:kim2005}. {\color{red}Both fluid and kinetic continuum approaches must further make assumptions regarding the VDF, one of the main impact parameters in magnetised plasma expansion \cite{b:ahedo2020}. {\color{blue}Hence}, numerical studies need to be extended to fully-kinetic \cite{b:difede2021,b:porto2019} or fluid-kinetic \cite{b:alvaro2021} approaches if the dynamics of a MN want to be treated self-consistently.} The fully-kinetic Particle-in-Cell (PIC) method represents the numerical strategy with the lowest level of assumptions. Both electron and ion populations are modelled as macro-particles, subject to the action of {\color{red}self-consistently computed} electric and magnetic fields, as well as particle collisions \cite{b:birdsall1991}.

{\color{blue}PIC simulations operate by necessity on a finite domain. Due to the ambipolar potential drop along the MN, and for the typical meso-thermal plume (electron thermal velocity greatly exceeds the ion drift velocity and ion thermal velocity). Most of the electron population will become trapped into the much-slower ion beam and reciprocate about the plume, with the point of their velocity inversion given by the equilibrium of their kinetic and potential energies \cite{b:merino2019iepc}. Since the computational domain is finite, the location of this reversal may exist beyond the domain, and an otherwise-trapped electron may be non-physically deleted upon reaching the domain boundary. The outcome is occurrence of the so-called ‘numerical pump instability’ \cite{b:briedaThesis}. So, since the response of confined electrons is non-local, the definition of consistent downstream (and lateral) boundary conditions is a challenging problem, not fully solved and is shared by unmagnetised plumes also.}

For this reason, simulations are usually stopped long before the ion beam reaches the outer boundaries.{\color{red} Thus, most results in the literature deal with short time-scale transient plume expansions in small domains \cite{b:levin2018, b:hu2017}. {\color{blue}Alternatively, to prevent the instability, an open model has been demonstrated where a virtual ion sink was implemented midway between the inlet and outer boundaries \cite{b:brieda2018}. Ions are absorbed by the sink while electrons can permeate through it, thus retaining the trapped electrons between the ion sink and the outer boundaries. Electrons are also reflected from the boundaries, based on a global charge conservation criterion. However, the sink must be located far from these boundaries, resulting in an unwelcome increase in the domain size.} To overcome this limitation, another charge-conserving boundary condition has been proposed \cite{b:levin2020}, where the number of electrons reflected at the open boundary is {\color{blue}determined so as to maintain a globally-neutral plasma}. Another approach, formulated to mimic the real physics, uses a current-free boundary condition \cite{b:li2019}. This has been demonstrated via simulations of both a non-magnetised plume \cite{b:li2019} and a MN \cite{b:chen2020}. {\color{blue}The methodology proposed \cite{b:li2019,b:chen2020} is well-founded concerning electron kinetics, but simplified conditions have been assumed for the solution of the electric field}: A zero-Neumann condition was imposed at the open boundary to solve the Poisson's equation.} Such a condition is appropriate only in the limit of an infinitely large domain that encompasses nearly all the potential fall that occurs in the plasma plume. For this reason, the authors of \cite{b:li2019} suggest ignoring the plasma dynamics in some portion of the domain near the outer boundaries (i.e., $\approx$20\%). Indeed, this boundary condition does not generally provide results which are domain independent.

{\color{red}This article presents a new electrostatic fully kinetic PIC model for MN plasma expansions. Boundary conditions are {\color{blue}introduced} to improve on previous works in terms of {\color{blue}both} electron kinetics and the Poisson's equation. Regarding the treatment of the electrons, a consistent approach has been defined to selectively reflect or absorb parts of the population crossing the open boundaries.} {\color{blue}The proposed approach mimics the partial reflection of electrons that would take place further downstream (outside of the domain), by enforcing the integral current-free condition along the outer boundaries and an energy-based reflection criterion on electrons. The total potential drop is self-consistently calculated to maintain the net-zero current and is included when determining an in-homogeneous non-stationary Robin boundary condition on the plasma potential. The result is a set of mutually consistent boundary conditions for performing steady-state full-PIC simulations of MN expansions that require an open boundary, which is sufficiently general such that both the plume kinetics, and plasma potential distribution, are independent of the computational domain size and in good agreement with experiments \cite{b:lafleur2011}.}

Section 2 summarises the key aspects of the PIC model and introduces the new boundary condition treatment. {\color{red}In Section 3 the capability to produce a stable steady-state plume and a {\color{blue}domain-independent solution is proven}. In section 4 the numerical approach has been benchmarked against experimental measures of plasma density and electrostatic potential \cite{b:lafleur2011}. In section 5 the validated approach has been exploited to investigate the plume expansion in a MN. The most relevant aspects analysed are: the presence of a radial potential well that {\color{blue}confines the plasma expansion}, the influence of the magnetic field intensity on the propulsive performance, and the evolution of the electron VDF.} The conclusions are then given in Section 6.

==> chap_2_MM.tex <==
\section{Numerical model}
%
\begin{figure}[!tb]
    \centering
    \includegraphics[width=\linewidth]{domainfinal.pdf}
    \caption{\color{red} ($I$) Thruster outlet, ($II$) axis of symmetry, and ($III$) external boundary. The electromagnet producing the MN is indicated at $r=R_c$. For Poisson equation, Dirichlet condition applies to ($I$), zero-Neumann to ($II$), and Robin to ($III$). Ions are absorbed on ($I$) and ($III$). Electrons are absorbed on ($I$) and selectively reflected on ($III$) based on an energy criterion. Particles are reflected on ($II$). $I_{i0}$ and $I_{e0}$ are the injected ion and electron currents. $I_{ib}$ and $I_{eb}$ are the ion and electron currents lost to ($III$). $\phi_\infty$ is the potential at infinity.}
    \label{fig:domainBC}
\end{figure}
%
The methodology has been developed by adapting the PIC code \textit{Starfish} which has been used previously to model Hall thruster channels \cite{b:brieda2012} and the plume of a magnetically-enhanced vacuum arc thruster \cite{b:zolotukhin2020}. An overview of the simulation domain is shown in Figure~\ref{fig:domainBC}. {\color{red}The computational domain is 2D-axisymmetric, namely the plume is solved along the radial ($r$) and the axial ($z$) directions of a cylindrical coordinate system aligned along the axis of the thruster. The azimuthal component ($\theta$) of the particles speed is computed and not assumed since Starfish is an axisymmetric 2D3V electrostatic-magnetostatic PIC code. The portion of the thruster where the plasma is produced has not been included in the computational domain since the scope of this work is to simulate the plume expansion. Instead, ions and electrons are injected through a boundary located in correspondence of the thruster outlet (labelled $I$ in Figure~\ref{fig:domainBC}). The boundary $II$ is the symmetry axis. The other boundaries, labelled as $III$, are treated as external surfaces. Hereafter, the subscripts $*$, $0$, $b$, and $\infty$ shall refer to plasma properties in an eventual reference source, at the thruster outlet (i.e., boundary $I$), at the external boundary ($III$), and at an hypothetical infinite distance from the thruster respectively. Likewise, the superscripts $+$ and $-$ shall refer to the forward and backward-marching components of the plasma flow. Boundary conditions are defined as if $I$ and $III$ were connected via a virtual capacitance which ensures equal ion and electron fluxes reach the infinity at steady-state; further details are provided in Sections 2.2-2.4.}

%
%
%
\subsection{Particle-in-Cell simulation}
{\color{red}The set of macro-particles $p = 1,...,N_p$ includes ions ($i$) and electrons ($e$). At the $n$-th time-step $t^n = n\Delta t$, positions are given as $\mathbf{r}^n_p=\langle z^n_p,r^n_p,0\rangle$, velocities $\mathbf{v}^n_p=\langle v_{pz}^n,v^n_{pr},v^n_{p\theta}\rangle$, masses ${m}_p$, and charges $q_p$. Particles dynamics are solved explicitly from the discrete equation of motion with the standard leap-frog Boris algorithm \cite{b:birdsall2005},}
%
\begin{equation}
\fl    \frac{\mathbf{v}^{n+1/2}_p -\mathbf{v}^{n-1/2}_p}{\Delta t}= \frac{q_p}{m_p}\left( \mathbf{E}^n_p+\frac{\mathbf{v}_p^{n+1/2}+\mathbf{v}_p^{n-1/2}}{2} \times \mathbf{B}_p\right)
\end{equation}
\begin{equation}
    \frac{\mathbf{r}^{n+1}_p-\mathbf{r}^{n}_p}{\Delta t}=\mathbf{v}^{n+1/2}_p, \qquad p = 1,...,N_p,
\end{equation}
%
where $\mathbf{E}^n_p$ is the electric field at $t^n$ in correspondence of the particle $p$, and $\mathbf{B}_p$ is the static background magnetic field. The movement of particles to new positions leads to a new distribution of charge density $\rho$, computed by scattering particles to the mesh nodes using a second-order Ruyten shape factor $S_p$ \cite{b:ruyten1993},
%
\begin{equation}
    \rho = \frac{1}{{V}}\sum_{p=1}^{N_p}{q_p w_p S_p},
    \label{eqn:rho}
\end{equation}
%
where $w_p$ is the macro-particle specific weight \cite{b:birdsall2005}, and ${V}$ the mesh cell of volume. The charge density is then used to solve for the self-consistent plasma potential $\phi$ according to the Poisson's equation, using an explicit successive over-relaxation (SOR) Gauss-Seidel scheme \cite{b:briedaThesis}.
%
\begin{equation}
    \epsilon_0\nabla^2\phi=-\rho,
\end{equation}
%
where $\epsilon_0$ is the vacuum permittivity. The electric field $\mathbf{E}=-\nabla\phi$ is then updated for the next time-step.

In order to reduce the computational burden, a scheme of numerical acceleration has been adopted. The vacuum permittivity is increased by a factor $\gamma^2$ and the mass of heavy particles is reduced by a factor $f$. {\color{red}This method does not require a scaled increase of the magneto-static field \cite{b:chen2020} which is particularly useful when handling a MN so as not to impose intractable conditions on the time-step required to resolve the electron gyromotion: for a typical $B_0 \sim \mathcal{O}(500G)$, $\Delta t \sim \mathcal{O}(10^{-12}s)$ \cite{b:birdsall2005}.} The relationships between the simulated and physical constants, provided by $f$ and $\gamma$, are shown in Eq.~\ref{eqn:scale}. The direct consequences of these factors on the Debye length and plasma frequency $\omega_{pe}=\sqrt{n_ee^2/m_e\epsilon_0}$ are provided in Eq.~\ref{eqn:scale2}. A summary on the scaling relationship on other parameters and retrieving physical results can be found in \cite{b:szabo}.
%
\begin{equation}
\tilde{m}_{i,n} \equiv \frac{{m_{i,n}}}{f} \qquad \tilde{\epsilon}_0 \equiv \gamma^2\epsilon_0
\label{eqn:scale}
\end{equation}
%
%
\begin{equation}
\tilde{\lambda}_D = \gamma\lambda_D \qquad \tilde{\omega}_{pe} = \frac{\omega_{pe}}{\gamma}
\label{eqn:scale2}
\end{equation}
%

%
%
%
\subsection{Boundary conditions on the Poisson equation}

The thruster outlet ($I$) is assumed at the reference potential $\phi_0=0$. The $r=0$ boundary ($II$) is symmetric, therefore the zero-Neumann condition $\partial\phi / \partial \hat{\mathbf{n}}=0$ is applied there. {\color{red}For what the external boundaries ($III$) are concerned, a Robin-type condition applies
%
\begin{equation}
    \frac{\partial\phi}{\partial\hat{\mathbf{n}}}+\frac{\hat{\mathbf{n}}_b\cdot{\mathbf{r}_b}}{\mathbf{r}_b\cdot\mathbf{r}_b}\left(\phi-\phi_\infty\right) = 0
    \label{eqn:robin}
\end{equation}
%
where $\mathbf{r}_b=\langle z_b-z_0, r_b-r_0\rangle$ is the vector distance from the centre of the thruster outlet ($I$) to the location on the external boundary ($III$), $\mathbf{\hat{n}}_b$ is the inward-pointing unit normal, and $\phi_\infty$ denotes the free-space plasma potential at infinity.} Eq.~\ref{eqn:robin} is a transparent condition modelling the $1/r$ monopole decay of the potential \cite{b:griffiths2013} far into the plasma $(\phi\rightarrow\phi_\infty, {\partial\phi}/{\partial\hat{\mathbf{n}}}\rightarrow0, \phi_\infty<0)$; its derivation is provided in the Appendix. {\color{red}The value of $\phi_\infty$ is self-consistently calculated during the simulation to ensure that, at the steady state, ion and electron current reaching the infinity are equal. The methodology adopted to derive $\phi_\infty$ is described in Section 2.4. Finally, it is worth noting that the condition expressed in Eq.~\ref{eqn:robin} is a generalization, in case of a finite size domain, of the commonly used zero-Neumann assumption \cite{b:chen2020}.}

%
%
%
\subsection{Boundary conditions on particle dynamics}

{\color{red}At each time step, ions and electrons are emitted from the thruster outlet boundary ($I$). For both species, a Maxwellian VDF is assumed; the reference temperature is $T_{e*}$ and $T_{i*}$ for electrons and ions respectively \cite{chen1999upper}. A drift velocity equal to the Bohm speed $c_{*} = \sqrt{k_B T_{e*}/m_i}$ is imposed along the $z$ direction \cite{b:martinez2015}. The resultant VDF reads
%
\begin{equation}
f_{e,i}^{+}(\mathbf{v}_{p}) = \sqrt{\frac{m_{e,i}}{2\pi T_{e,i*}}}\exp \left(-\frac{m_{e,i}}{2T_{e,i*}}(\mathbf{v}_{p}-\mathbf{u}_{0})^2 \right)
\label{eqn:f}
\end{equation}
%
where $\mathbf{u}_{0} = \langle c_{*},0,0\rangle$. At the thruster outlet ($I$) a condition only on the forward-marching particles ($v_{pz}>0$) can be imposed since the dynamics of the backward-marching particle is an output of the simulation which strongly depends on the value of $\phi_\infty$ (see Section 2.4). In this regard, any backward-marching electrons (and ions) returning to boundary ($I$) are absorbed. In fact, once inside the source where the density is high and collisions are frequent, a particle will become re-equilibrated with the surrounding plasma and lose all its memory when it is re-injected into the beam \cite{b:lafleur2015,chen1999upper}. $T_{e,i*}$ represent the expected plasma properties within the source. They are not necessarily equal to the temperature computed at the thruster outlet since the dynamics of the backward-marching species cannot be imposed \textit{a priori} (e.g., $f_{e,i}^{-}$ might be non-Maxwellian).} At the symmetry plane ($II$), all particles are specularly reflected.

Since ions are accelerated outward the simulation domain by the ambipolar electric field \cite{b:lafleur2015}, no special treatment is required at the external boundaries ($III$); therefore ions reaching them are simply absorbed. For electrons, the behaviour is not as straightforward. Generation of a stable steady-state plume without altering the electron kinetics requires an energy-based treatment for the electrons \cite{b:li2019}. {\color{red} From a physical standpoint, two separate populations of electrons can be identified depending on their total energy, namely bounded and free (see Figure~\ref{fig:electrons}). The former are the less energetic electrons that cannot cross the potential drop that occurs across the plume, namely bounded electrons are forced to be turned back to the plasma source at a certain distance from the thruster. The latter are the electrons that have energy enough to cross the potential barrier and to escape at an infinite distance from the thruster. Specifically, assuming a collision-less, steady-state, and axisymmetric electric field, the total energy of each electron can be defined as 
%
\begin{equation}
    E_e=\frac{1}{2}m_e(v_{ez}^2+v_{er}^2+v_{e\theta}^2)-e\phi(\mathbf{r})
    \label{eqn:energy}
\end{equation}
%
where $E_e$ is a constant conserved quantity of the motion. By the definition $\phi_0=0$, $E_e$ is identical to the initial injected kinetic energy, namely $E_e>0$. From energy conservation, bounded electrons are characterized by $E_e<|e\phi_\infty|$, while for free electrons $E_e\geq|e\phi_\infty|$ (see Figure~\ref{fig:electrons}).}
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{electrons.pdf}
    \caption{\color{red}Illustration of the potential drop ($\phi$) across the axis of the plume ($z$). The trajectories of bounded and free electrons are depicted.}
    \label{fig:electrons}
\end{figure}
%
{\color{red}From these considerations, the following boundary conditions are defined.} When an electron reaches an outer boundary node $b$, it's kinetic energy is taken as $KE_{eb}=\frac{1}{2}m_e|\mathbf{v}_{eb}|^2$, and then compared to the trapping potential $PE_{b}=e(\phi_\infty-\phi_b)$. 
\begin{itemize}
    \item If $KE_{eb}<PE_{b}$ the electron is bounded, so it is reflected back with velocity $-\mathbf{v}_{eb}$.
    \item Else, it is a free electron to be removed from the domain.
\end{itemize}  
This boundary condition therefore allows the highest-energy electrons to escape, but retains the physical proportion of the bounded population ensuring stability \cite{b:li2019,b:brieda2018}. Finally, the key assumptions in this energy-based boundary condition are, firstly, that the plasma is collision-less downstream of the external boundaries and that, beyond the domain, the magnetisation is not so strong as to induce reflection of highly energetic electrons \cite{b:martinez2015}.

%
%
%
\subsection{Capacitive circuit} 

{\color{red}In order to enforce the current-free condition, a sufficient number of electrons shall be reflected each time-step such that a zero net global current is established. The number of reflected electrons is dependant on the potential barrier $|e\phi_\infty|$ according the the energy-based criterion discussed in Section 2.3. Therefore, the value of $\phi_\infty$ is self-consistently controlled via a virtual capacitance $C$. The resultant control algorithm reads}
%
\begin{equation}
    \phi_\infty^{n+1}=\phi_\infty^n+\frac{1}{C}(I_{ib}^nf^{-0.5}+I_{eb}^n)\Delta t,
    \label{eqn:control}
\end{equation}
%
where $I_{ib}$ and $I_{eb}$ are the sum ion and electron current leaving the external boundary, with the factor $f^{-0.5}$ scaling down the ion current in accordance with the applied mass correction \cite{b:szabo}. The value of $C$ must be carefully chosen according to a compromise between fast convergence of $\phi_\infty$ and stability of the Poisson solver {\color{red}(see the sensitivity analysis reported in Section 3.1).} 
This method ensures that the system evolves self-consistently and inherently guarantees that once at steady-state, the ion and electron currents are equal ($I_{ib}=-I_{eb}$) at the outer boundaries. The initial value of $\phi_\infty$ {\color{red}($\phi_\infty^0$)} is set according to the theoretical value obtained by assuming a current-free condition at the thruster outlet, tha absence of magnetic field, and the energy conservation \cite{c:DiFede2021,b:SPPIC}. For the Maxwellian electron population given by Eq.~\ref{eqn:f}, the analytical result reads
%
\begin{equation}
\fl 1+erf\sqrt{\frac{-e\phi_\infty^0}{T_{e*}}}-\sqrt{\frac{-2e\phi_\infty^0}{\pi T_{e*}}}exp\left(\frac{e\phi_\infty^0}{T_{e*}}\right) = \frac{4u_{i0}}{\bar{v}_{e*}},
\label{eqn:phi0}
\end{equation}
%
where $\bar{v}_{e*}=\sqrt{8k_BT_{e*}/\pi m_e}$ is the mean reference electron velocity. For $u_{i0}=c_{*}$ with Xenon, Eq.~\ref{eqn:phi0} yields $e\phi_\infty^0\sim -6.4T_{e*}$.

{\color{red}Controlling only the value of $\phi_\infty$ by means of Eq.~\ref{eqn:control} is not sufficient to implement a self-consistent circuit condition. The total current leaving from the external boundaries ($III$) shall be re-injected into the domain via the thruster outlet ($I$) \cite{b:brieda2018}. Moreover, the emitted electron current ($I_{e0}^+$) shall be controlled in order to enforce the quasi-neutrality condition at boundary ($I$), namely
%
\begin{equation}
n_{i0} = n_{e0}^+ + n_{e0}^-
\label{eqn:quas-neutr}
\end{equation}
%
where $n_{i0}$ is the ion density at the thruster outlet, $n_{e0}^+$ is the electron density associated to forward-marching electrons, and $n_{e0}^-$ to backward-marching electrons. Being $n_{e0}^-$ unknown \textit{a priori}, Eq.~\ref{eqn:quas-neutr} can be satisfied at the steady state only adjusting $I_{e0}^+$ and, in turn, $n_{e0}^+$. From these considerations, the following conditions are imposed to the particles injected from boundary ($I$). Ions are emitted with a constant current given by $I_{i0} = en_{*}c_{*}A_0$, where $A_0$ is the area of the thruster outlet, and $n_{*}$ the reference plasma density in the source. The emitted electron current is updated each time step according to 
%
\begin{equation}
{I_{e0}^+}^{n+1} = (I_{ib}^nf^{-0.5}+I_{eb}^n) + \frac{n_{i0}^n}{n_{e0}^n}{I_{e0}^+}^{n}
\label{eqn:QN}
\end{equation}
%
where the first term completes the circuit and the second enforces the quasi-neutrality. This condition guarantees that quasi-neutrality and current-free conditions are respected at the steady state. A similar control strategy has not been imposed to ions since $I_{i0} \equiv I^+_{i0}$, whereas $I_{e0}^+ \neq I_{e0}$. Considering that electrons are Maxwellian, the initial value of the current is set as ${I_{e0}^+}^0=-en_{*}(\bar{v}_{e*}/4+c_{*})A_0$.}

It is prudent to state that $\phi_\infty$ and $I_{e0}^+$ are numerically stored on the order of the inverse plasma frequency as their moving average, therefore minimising any PIC noise from the fluctuations in their value. There thus exists a fully-consistent relationship between the current flowing from the plasma source to the external boundaries $I_{ib}=-I_{eb}$, the potential drop $\phi_\infty$ and the macroscopic plume solution. It is established via the boundary condition of Eq.~\ref{eqn:robin}, the electron energy reflection condition, and the capacitive circuit control of Eq.~\ref{eqn:control} and Eq.~\ref{eqn:QN}.

%
%
%
\subsection{Performance indicators}
The thrust $F$ is given by the axial flux integral
%
\begin{equation}
F = \int_{S_b} \sum_k \left(n_k m_k v_{kz}\mathbf{v}_k + p_k\hat{\mathbf{z}} \right) \cdot\hat{\mathbf{n}}~dS_b,
\label{eqn:thrust}
\end{equation}
%
where the two terms correspond to the species momentum flux and pressure $p_k=n_k k_B T_k$ respectively, for $k=i,e$. $S_b$ is the external boundary ($III$) surface. The specific impulse $I_{sp}$ is then 
%
\begin{equation}
I_{sp} = \frac{F}{\dot{m}g_0},
\end{equation}
%
with $\dot{m}$ the propellant mass flow rate and $g_0$ the standard gravitational acceleration.





==> chap_2_SA.tex <==
\section{Physical and numerical model}
%
\begin{figure*}[!tb]
    \centering
    \includegraphics[width=\linewidth]{domainfinal.pdf}
    \caption{\color{red} ($I$) Thruster outlet, ($II$) symmetric boundary, and ($III$) open boundary. The electromagnet producing the MN is indicated at $r=R_c$. For the Poisson's equation, a Dirichlet condition applies to ($I$), zero-Neumann to ($II$), and Robin to ($III$). Ions are absorbed on ($I$) and ($III$). Electrons are absorbed on ($I$) and selectively reflected on ($III$) based on an energy criterion. Particles are specularly reflected on ($II$). $I_{i*}$ and $I_{e*}$ are the injected ion and electron currents. $I_{iB}$ and $I_{eB}$ are the ion and electron currents lost to ($III$). $\phi_\infty$ is the potential at infinity.}
    \label{fig:domainBC}
\end{figure*}
%

The model has been developed by adapting {\color{blue}the fully kinetic axisymmetric 2D3V PIC code} \textit{Starfish}, which has been used previously to model Hall thruster channels \cite{b:brieda2012} and the plume of a magnetically-enhanced vacuum arc thruster \cite{b:zolotukhin2020}. An overview of the simulation domain is shown in Figure~\ref{fig:domainBC}. {\color{red}{\color{blue}The domain consists of a cylindrical 2D $(z,r)$ region corresponding to a plane at $\theta = 0$}. {\color{blue}The plasma source has not been included since the scope of this work is to simulate purely the plume expansion}. Instead, ions, electrons and neutrals are injected through a boundary corresponding to the thruster outlet ($I$). The external boundaries ($III$) are treated as open to vacuum, connected to the thruster outlet ($I$) via a virtual free-space capacitance which ensures equal ion and electron current streams to the infinity at steady-state. This allows the plasma source to float relative to the surroundings, similar to what happens in the operation of the thruster in space; further details are provided in Sections 2.2-2.4. Boundary ($II$) is the axis of symmetry.

{\color{blue}Hereafter, the subscripts $*$, $0$, $b$ and $\infty$ shall refer to properties within the plasma source (reference), at the thruster outlet boundary ($I$), at the open boundaries ($III$) and at the virtual infinity respectively. {\color{blue}The subscript $B$ shall refer to the integral sum of local properties along the open boundaries, i.e. $B=\sum b$.} Likewise, the superscripts $+$ and $-$ shall refer to the forward and backward-marching components of the plasma properties.}}

%
%
%
\subsection{Particle-in-Cell simulation}
{\color{red}The set of macro-particles $p = 1,...,N_p$ with positions $\mathbf{r}^n_p=\langle z^n_p,r^n_p,0\rangle$, velocities $\mathbf{v}^n_p=\langle v_{pz}^n,v^n_{pr},v^n_{p\theta}\rangle$, masses ${m}_p$, and charges $q_p$, sample the continuum phase space of ions $i$, electrons $e$ and neutrals $g$ at the $n$-th time-step $t^n = n\Delta t$. The particle Newton-Lorentz motion is solved explicitly with the standard leap-frog Boris algorithm \cite{b:birdsall2005},}
%
\begin{eqnarray}
 & \frac{\mathbf{v}^{n+1/2}_p -\mathbf{v}^{n-1/2}_p}{\Delta t}=\nonumber\\  &\qquad \frac{q_p}{m_p}\left( \mathbf{E}^n(\mathbf{r}_p^n)+\frac{\mathbf{v}_p^{n+1/2}+\mathbf{v}_p^{n-1/2}}{2} \times \mathbf{B}(\mathbf{r}_p^n)\right) 
 \end{eqnarray}
\begin{equation}
    \frac{\mathbf{r}^{n+1}_p-\mathbf{r}^{n}_p}{\Delta t}=\mathbf{v}^{n+1/2}_p, \qquad p = 1,...,N_p,
\end{equation}
%
where $\mathbf{E}^n$ is the electric field, and $\mathbf{B}$ is the static background magnetic field. The movement of particles to new positions leads to a new distribution of charge density $\rho=n_i-n_e$, where $n_i$ is the ion density and $n_e$ is the electron density, computed by scattering particles to the mesh nodes using a second-order Ruyten shape factor $S_p$ \cite{b:ruyten1993},
%
\begin{equation}
    \rho = \frac{1}{{V}}\sum_{p=1}^{N_p}{q_p w_p S_p},
    \label{eqn:rho}
\end{equation}
%
where $w_p$ is the macro-particle specific weight \cite{b:birdsall2005}, and ${V}$ the mesh cell volume. The charge density is then used to solve for the self-consistent plasma potential $\phi$ according to the Poisson's equation, using an explicit successive over-relaxation (SOR) Gauss-Seidel scheme \cite{b:briedaThesis}.
%
\begin{equation}
    \epsilon_0\nabla^2\phi=-\rho,
\end{equation}
%
where $\epsilon_0$ is the vacuum permittivity. The electric field $\mathbf{E}=-\nabla\phi$ is then updated for the next time-step. To comply with typical PIC stability criteria, the mesh spacing is kept below the expected Debye length $\lambda_D = \sqrt{\epsilon_0k_BT_e/n_ee^2}$, where $k_B$ is the Boltzmann constant and $e$ is the elementary charge.

In order to reduce the computational burden, a numerical acceleration scheme has been adopted: The vacuum permittivity is increased by a factor $\gamma^2$ and the mass of heavy species reduced by a factor $f$. {\color{red}This method does not require a scaled increase of the magneto-static field \cite{b:chen2020}, which is particularly useful when handling a MN expansion so as not to impose intractable conditions on the time-step required to resolve the electron gyroperiod $\omega_{ce}=e|\mathbf{B}|/m_e$.} The relationships between the simulated and physical constants, provided by $f$ and $\gamma$, are shown in Eq.~\ref{eqn:scale}. The direct consequences of these factors on the Debye length and plasma frequency $\omega_{pe}=\sqrt{n_ee^2/m_e\epsilon_0}$ are provided in Eq.~\ref{eqn:scale2}. A summary on the scaling relationship on other parameters and retrieving physical results can be found in \cite{b:szabo}.
%
\begin{equation}
\tilde{m}_{i,n} \equiv \frac{{m_{i,n}}}{f} \qquad \tilde{\epsilon}_0 \equiv \gamma^2\epsilon_0
\label{eqn:scale}
\end{equation}
%
%
\begin{equation}
\tilde{\lambda}_D = \gamma\lambda_D \qquad \tilde{\omega}_{pe} = \frac{\omega_{pe}}{\gamma}
\label{eqn:scale2}
\end{equation}
%
Depending on the plasma parameters and magnetic field strength, the computational time should be reduced by a a factor $\gamma^2\sqrt{f}$ or $\gamma^3\sqrt{f}$.

Collision processes between ions, electrons and neutrals are simulated using a combination of Direct Simulation Monte Carlo (DSMC) \cite{b:bird1998} and Monte Carlo Collision (MCC) \cite{b:birdsall1991} methods. All simulations contained within this article consider six different collision processes: electron-electron Coulomb scattering, electron-ion Coulomb scattering, electron-neutral elastic scattering, ion-neutral elastic scattering, ion-neutral charge exchange, and neutral-neutral elastic scattering. All relevant cross-sections are recovered from the LXCat database \cite{LXCat}. 
%
%
\subsection{Boundary conditions on the Poisson's equation}

The thruster outlet ($I$) is given the reference potential $\phi_0=0$. The $r=0$ boundary ($II$) is symmetric, therefore the zero-Neumann condition $\partial\phi / \partial \hat{\mathbf{n}}=0$ is applied there. {\color{blue}Concerning the open boundaries ($III$), a non-stationary Robin-type condition is introduced of the form
%
\begin{equation}
    \frac{\partial\phi}{\partial\hat{\mathbf{n}}}\bigg|^n_b+\frac{\hat{\mathbf{n}}_b\cdot{\mathbf{r}_b}}{\mathbf{r}_b\cdot\mathbf{r}_b}\left(\phi^n_b-\phi^n_\infty\right) = 0
    \label{eqn:robin}
\end{equation}
%
where $\mathbf{r}_b=\langle z_b-z_0, r_b-r_0\rangle$ is the vector distance from the centre of the thruster outlet ($I$) to the location on the open boundary ($III$), $\mathbf{\hat{n}}_b$ is the inward-pointing unit normal, and $\phi_\infty$ denotes the plasma potential at infinity.}

Eq.~\ref{eqn:robin} is a transparent condition modelling the $1/r$ monopole decay of the potential \cite{b:griffiths2013} far into the plasma $(\phi\rightarrow\phi_\infty, {\partial\phi}/{\partial\hat{\mathbf{n}}}\rightarrow0, \phi_\infty<0)$; its derivation is provided in the Appendix. The condition inherently provides the physical potential drop $|\phi_\infty|$ at $\mathbf{r}=\infty$. {\color{blue}The procedure adopted to self-consistently calculate $\phi_\infty$ ensures that, at steady-state, ion and electron currents reaching the infinity are equal; this is described in section 2.4. Finally, it is worth noting that the condition expressed in Eq.~\ref{eqn:robin} is a generalisation of the commonly used zero-Neumann assumption \cite{b:chen2020} for the case of a finite domain.}

%
%
%
\subsection{Boundary conditions on particle kinetics}

{\color{red}At each time step, ions, electrons and neutrals are emitted from the thruster outlet boundary ($I$). For all species, a Maxwellian VDF is assumed; the reference temperatures are $T_{p*}$ \cite{chen1999upper}. A drift velocity equal to the Bohm speed $c_{*} = \sqrt{k_B T_{e*}/m_i}$ is imposed along the $z$ direction \cite{b:martinez2015} for both ions and electrons. The resultant generic VDF reads
%
\begin{eqnarray}
& f_{p}^{+}(\mathbf{v}_{p}) = \sqrt{\frac{m_{p}}{2\pi T_{p*}}}\exp \left(-\frac{m_{p}}{2T_{p*}}(\mathbf{v}_{p}-\mathbf{u}_{p})^2 \right)H(v_{pz}) \nonumber\\ &~
\label{eqn:f}
\end{eqnarray}
%
where $\mathbf{u}_{i,e} = \langle c_{*},0,0\rangle$. Neutrals possess diffusion drift velocity $\mathbf{u}_{g} = \langle \bar{v}_n/4,0,0\rangle$, where $\bar{v}_n=\sqrt{8k_BT_{n*}/\pi m_g}$. The Heaviside $H$ makes the distribution one-sided, since only forward-marching distributions ($v_{pz}>0$) can be imposed. The backward-marching distributions $f^-_p$ are an output of the simulation which strongly depends on the steady-state value of $\phi_\infty$ (see Section 2.4). In this regard, any backward-marching electrons (and ions or neutrals) returning to boundary ($I$) are absorbed. In fact, once inside the source where the density is high and collisions are frequent, an electron will become re-equilibrated with the source plasma and lose all its memory when it is re-injected into the beam \cite{b:lafleur2015,chen1999upper}. The values of $T_{p*}$ represent the expected plasma properties within the source; they are not necessarily equal to the final temperature at the thruster outlet $T_{p0}$ since the dynamics of the backward-marching species are not known \textit{a priori} (e.g., $f_{e}^{-}$ might be non-Maxwellian).} At the symmetry plane ($II$), all particles are specularly reflected.

Since ions are accelerated outward by the ambipolar electric field \cite{b:lafleur2015}, no special treatment is required at the open boundaries ($III$); therefore ions reaching them are simply absorbed. Neutrals are also absorbed. For electrons, the behaviour is not as straightforward. Generating a stable steady-state plume without altering the electron kinetics requires an energy-based treatment \cite{b:li2019}. {\color{red} Physically, two separate populations of electrons can be identified depending on their total energy, namely trapped and free. The former are the less energetic electrons that cannot cross the potential drop that occurs across the plume. The trapped electrons are forced to turn back to the plasma source at a certain distance downstream. The free population are the electrons that have energy enough to cross the potential barrier and thus escape to infinity. Assuming a collision-less, steady-state, and axisymmetric electric field, the total energy of each electron can be defined as 
%
\begin{equation}
    E_e=\frac{1}{2}m_e(v_{ez}^2+v_{er}^2+v_{e\theta}^2)-e\phi(\mathbf{r})
    \label{eqn:energy}
\end{equation}
%
where $E_e$ is a constant conserved quantity of the motion. By the definition $\phi_0=0$, $E_e$ is identical to the initial injected kinetic energy, that is $E_e>0$. From energy conservation, trapped electrons are characterised by $E_e<|e\phi_\infty|$, while for free electrons $E_e\geq|e\phi_\infty|$.}
%
{\color{red}From these considerations, the following boundary conditions are defined.} When an electron reaches an open boundary node $b$, it's kinetic energy is taken as $KE_{eb}=\frac{1}{2}m_e|\mathbf{v}_{eb}|^2$, and then compared to the trapping potential $PE_{b}=e(\phi_\infty-\phi_b)$. 
\begin{itemize}
    \item If $KE_{eb}<PE_{b}$ the electron is trapped, so it is reflected back with velocity $-\mathbf{v}_{eb}$.
    \item Else, it is a free electron to be removed from the domain.
\end{itemize}  
This boundary condition therefore allows the highest-energy electrons to escape, but retains the physical proportion of the trapped population, ensuring stability \cite{b:li2019,b:brieda2018}. Finally, the key assumptions in this energy-based boundary condition are, firstly, that the plasma is collision-less downstream of the open boundaries and that, beyond the domain, the magnetisation is not so strong as to induce reflection of highly energetic electrons \cite{b:martinez2015}.

%
\subsection{Capacitive circuit} 

{\color{blue} The value of $\phi_\infty$ is a non-stationary unknown and must be calculated self-consistently as part of the solution. There exists a current-voltage curve $dI_\infty/d|\phi_\infty|>0$ between the net beam current streaming to infinity $I_\infty=I_{i\infty}+I_{e\infty}$ and the free-space potential. From the energy-based criterion discussed in Section 2.3, there is a value of $\phi_\infty$ that reflects sufficient electrons to maintain a current-free plume. Therefore, the value of $\phi_\infty$ is self-consistently controlled via a virtual free-space capacitance $C$. The resultant control algorithm reads}
%
\begin{equation}
    \phi_\infty^{n+1}=\phi_\infty^n+\frac{1}{C}(I_{iB}^n{f}^{-0.5}+I_{eB}^n)\Delta t,
    \label{eqn:control}
\end{equation}
%
where $I_{iB}$ and $I_{eB}$ are the sum ion and electron currents leaving the external open boundaries ($III$), with the factor ${f}^{-0.5}$ scaling down the ion current in accordance with the applied mass factor \cite{b:szabo}. The value of $C$ must be carefully chosen according to a compromise between fast convergence of $\phi_\infty$ and stability of the Poisson solver {\color{red}(see the sensitivity analysis reported in Section 3.1).} This method ensures that the system evolves self-consistently and inherently guarantees that, once at steady-state, the ion and electron currents are equal ($I_{iB}=-I_{eB}$) at the open boundaries ($III$), and therefore also at the infinity.
%
The initial value of $\phi_\infty$ {\color{red}($\phi_\infty^0$)} is set according to the theoretical value obtained by assuming a current-free condition at the thruster outlet, the absence of a magnetic field, and electron energy conservation \cite{c:DiFede2021,b:SPPIC}. For the Maxwellian population given by Eq.~\ref{eqn:f}, the analytical result reads
%
\begin{eqnarray}
 &\frac{4u_{i0}}{\bar{v}_{e*}}=1+erf  \sqrt{\frac{-e\phi_\infty^0}{T_{e*}}} -\sqrt{\frac{-2e\phi_\infty^0}{\pi T_{e*}}}exp\left(\frac{e\phi_\infty^0}{T_{e*}}\right) \nonumber\\ &~
\label{eqn:phi0}
\end{eqnarray}
%
where $\bar{v}_{e*}=\sqrt{8k_BT_{e*}/\pi m_e}$ is the mean reference electron velocity. For $u_{i0}=c_{*}$ with xenon, Eq.~\ref{eqn:phi0} yields $e\phi_\infty^0\sim -6.4T_{e*}$.

{\color{red}Controlling only the value of $\phi_\infty$ by means of Eq.~\ref{eqn:control} is not in itself sufficient to implement a self-consistent circuit condition. The total current leaving the open boundaries ($III$) must be re-injected into the domain via the thruster outlet ($I$) \cite{b:brieda2018}. Moreover, the injected electron current ($I_{e*}$) is controlled in order to enforce the quasi-neutrality condition at boundary ($I$), namely
%
\begin{equation}
n_*=n_{i0} = n_{e0}^+ + n_{e0}^-
\label{eqn:quas-neutr}
\end{equation}
%
Being $n_{e0}^-$ unknown \textit{a priori}, Eq.~\ref{eqn:quas-neutr} can be satisfied at the steady-state by adjusting $I_{e*}$ and, in turn, $n_{e0}^+$. From these considerations, the following conditions are imposed to the particles injected from boundary ($I$). Ions are emitted with a constant current given by $I_{i*} = en_{*}c_{i*}A_0$, where $A_0$ is the area of the thruster outlet. The emitted electron current is updated each time step according to 
%
\begin{equation}
{I_{e*}}^{n+1} = (I_{iB}^n+I_{eB}^n) + \frac{n_{i0}^n}{n_{e0}^n}{I_{e*}}^{n}
\label{eqn:QN}
\end{equation}
%
where the first term completes the circuit and the second enforces the quasi-neutrality. This condition guarantees that quasi-neutrality and current-free conditions are respected at the steady-state. A similar control strategy has not been imposed to ions since $I_{i* }\equiv I_{i0} \equiv I^+_{i0}$, whereas $I_{e*} \equiv I_{e0}^+ \neq I_{e0}$. Considering that electrons are Maxwellian, the initial value of the current is set as ${I_{e*}}^0=-en_{*}(\bar{v}_{e*}/4+c_{i*})A_0$.} The neutral flux is imposed as $\Gamma_{n*}=n_{g*}\bar{v}_g/4A_0$.

It is prudent to state that $\phi_\infty$ and $I_{e*}$ are numerically stored as their moving average, on the order of the inverse plasma frequency, therefore minimising any PIC noise from the fluctuations in their value. There thus exists a fully-consistent relationship between the current flowing from the plasma source to the external boundaries $I_{iB}=-I_{eB}$, the potential drop $\phi_\infty$ and the macroscopic plume solution. It is established via the boundary condition of Eq.~\ref{eqn:robin}, the electron energy reflection condition, and the capacitive circuit control of Eq.~\ref{eqn:control} and Eq.~\ref{eqn:QN}.





==> chap_3_MM.tex <==
\section{\color{red}Verification of the numerical methodology}

{\color{red}This section demonstrates the numerical robustness of the proposed new boundary conditions. The investigation is divided into two parts, first the stability at steady state of the new model is compared with classical open outflow boundary conditions \cite{b:levin2018, b:hu2017}.} The latter consist in constant electron current emitted from the plasma source, absorption of macro-particles reaching the external boundary ($III$) and the zero-Neumann condition on the Poisson equation. {\color{red}Second, a domain independence study is accomplished evaluating both the plasma parameters (e.g., density and potential) and the propulsive performance (e.g., thrust) in respect to the axial and the radial domain dimensions.}

Table~\ref{tab:verparams} summarizes the physical and numerical parameters which are used, unless otherwise specified, throughout the simulations presented within this section. {\color{red}The radius of the thruster outlet ($R_0$), the propellant utilized (i.e., xenon) and the mass flow rate are typical of a low-power (i.e., 50 W power range) HPT \cite{b:manente2019}. The reference plasma properties assumed within the source are in agreement with the validated results provided by numerical codes handling the same class of thrusters \cite{b:magarotto2020,b:magarotto2020_3}. A purely divergent MN is produced by an electromagnet \cite{pottinger2011performance} of radius $R_c$ and located in correspondence of the thruster outlet ($z=0$).} Figure~\ref{fig:b_field} illustrates the magnetic field topology ($\mathbf{B}$) on the nominal simulation domain {\color{red}The intensity of the magnetic field is defined in terms of its value at the magnetic throat, namely $B_0=|\mathbf{B}(0,0)|$.} In the following, the case $B_0=0$ is referred to as ``unmagnetised'', $B_0=100G$ as ``low-magnetisation'', and $B_0=500G$ as ``high-magnetisation''.
%
\begin{figure}[!b]
    \centering
    \includegraphics[width=\linewidth]{dsmcBfield.eps}
    \caption{\color{red}(a) Normalised magnetic field magnitude $|\mathbf{B}|/B_0$. The electromagnet has radius $R_c=3.6R_0$. (b) Neutral density $n_g$ from the DSMC pre-simulation.}
    \label{fig:b_field}
\end{figure}
%

{\color{red}The scaling factors applied to the ion mass and the vacuum permittivity are $f=250$ \cite{b:szabo} and $\gamma=26.9$ respectively. The latter value is chosen so that $R_0=20\tilde{\lambda}_{D*}$, where $\tilde{\lambda}_{D*}$ is the scaled value of the Debye length in the source. This choice influences the resolution of the mesh since, according to the stability criteria for PIC simulations \cite{b:birdsall2005}, the size of the mesh is equal to $\tilde{\lambda}_{D*}$, namely the thruster outlet is resolved with 20 cells. The domain spans $L_z=25R_0$ in length and $L_r=10R_0$ in height, namely it is meshed with $10^5$ structured squared cells. The time-step adopted satisfies $\Delta t \omega_{ce0}=0.35$, where $\omega_{ce0}$ is the electron gyro-frequency at the thruster outlet. In this way, the electron gyro-motion is resolved in all the domain and the stability criterion on the resolution of the ``scaled'' plasma oscillation \cite{b:birdsall2005} is satisfied too (see Table~\ref{tab:verparams}). The Poisson's equation is solved every $0.286\tilde{\omega}_{p*}/\omega_{ce0}$ iterations \cite{b:birdsall2005} where $\tilde{\omega}_{p*}$ is the scaled plasma frequency.} Macro-particle weights are selected so as to maintain an average numeber of macro-particles per cell above 10 at the steady-state, {\color{red}as a result $w_p\approx10^6$.} The steady-state is characterised by the number of macro-particles leaving the domain matching the number of newly born macro-particles at the thruster outlet. Specifically, the change in the number of macro-particles between two consecutive iterations shall be less than 0.01\%.
%
\begin{table*}[!tb]
\caption{\label{tab:verparams} \color{red} Simulation parameters.}
\lineup
\centering
\begin{indented}
\item[]\begin{tabular}{@{}llll@{}}
\br
Parameter                          &                               & Unscaled             & Scaled              \\ \mr
Thruster Outlet Radius               & $R_0$ [m]                  & 0.010                   & -                    \\
Ion Mass (Xe)                      & $m_i$ [kg]                  & $2.18\times10^{-25}$ & $5.45\times10^{-23}$ \\
Propellent Mass Flow Rate          & $\dot{m}$ [mg/s]        & 0.200                & 3.16                 \\
Reference Plasma Density           & $n_{*}$ [m$^{-3}$]              & $8\times10^{17}$     & -                    \\
Reference Ion Temperature          & $T_{i*}$ [K]               & 298                  & -                    \\
Reference Electron Temperature     & $T_{e*}$ [eV]              & 5                    & -                    \\
Reference Bohm Speed              & $c_{*}$ [m/s]         & 1920                 & 30310                \\
Ion Current                        & $I_{i0}$ [A]                & 0.0770             & $1.22$               \\
Electromagnet Radius                & $R_c$ [mm]                  & 38                   & -                    \\
Throat Magnetic Field Strength     & $B_0$ [G]                   & $0-1000$              & -                    \\ \mr
Axial Domain Length                & $L_z$ [m]                  & 0.250                  & -                    \\
Radial Domain Length               & $L_r$ [m]                  & 0.100                  & -                    \\
Simulated Time                     & $T$ $[\mu s]$                 & -                    & 50                   \\
Scaling mass factor                & $f$                       &  -                      & 250\\
Scaling permittivity factor        & $\gamma$                       &  -                      & 26.9\\
Reference Debye Length             & $\lambda_{D*}$ [mm]        & 0.0186             & $0.500$              \\
Reference Plasma Frequency         & $\omega_{p*}$ [rad/s] & $8.02\times10^{10}$  & $2.98\times10^{8}$   \\
Electron Gyro-Frequency$^a$          & $\omega_{ce0}$ [rad/s]  & $1.10\times10^{10}$  & -                  \\
Number of Axial Cells              & $N_z$                         & -                    & 500                  \\
Number of Radial Cells             & $N_r$                         & -                    & 200                  \\ 
Number of Time-steps$^a$           & $N_t$                         & -                    & $1.58\times10^6$     \\
Macroparticle weight               & $w_p$                         & $\approx 10^6$                    & -     \\
\br
\end{tabular}
\item[] $^a$ ``Low-magnetisation'' case.
\end{indented}
\end{table*}

%
%
%
\subsection{Steady state}

\subsubsection{\color{red}Boundary conditions}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{bctime.eps}
    \caption{\color{red}(a) Total number of macro-particles $N_p$ for ions (\fullcircle) and electrons (\textcolor{red}{\full}) in the new model, and ions (\dashed) and electrons (\textcolor{red}{\dashed}) for the open outflow conditions; (b) free-space potential drop $\phi_\infty$; (c) net current $I_0$ at the thruster outlet ($I$); (d) net current $I_b$ at the external boundary ($III$); and (e) thrust $F$. All quantities are depicted in function of the simulation time $t$.}
    \label{fig:oneDtest}
\end{figure}
%
{\color{red}The stability of the new model is assessed in case of a collisionless and unmagnetised plume (i.e., $B_0=0$) since results can be more easily compared to theoretical values. The time-step is $\Delta t = 0.05/\tilde{\omega}_{p*} = 1.68\times10^{-10}s$.} Figure~\ref{fig:oneDtest}(a) gives the evolution of the macro-particle count for both the new model and the open outflow conditions. Although both simulations start with a similar growth in ion count during the transient, the electron count peaks around $8.5\mu s$ with the open outflow boundary. Despite the number of ions continuing to increase, the electron count decreases, resulting in a growing charge imbalance. This eventually results in the formation of a virtual anode \cite{b:brieda2018,b:briedaThesis} around $20\mu s$, which is followed by mild ion loss. The vast majority of electrons are lost to the boundary, thus the simulation collapses; this is the ``vacuum pump'' instability \cite{b:brieda2018,b:briedaThesis}. No such instability is observed with the new model. The electron and ion populations closely trend each other. Steady state is achieved near $21\mu s$, and the ion and electron counts remain invariant for the reminder of the simulation.

To illustrate that the new model can self-consistently predict the potential drop across the plume ($\phi_\infty$), Figure~\ref{fig:oneDtest}(b) plots its value against the simulation time. The trend depicted mimics the voltage seen across the charging-discharging cycle of a capacitor \cite{b:griffiths2013}. Indeed, from Figure~\ref{fig:oneDtest}(c), the presence of large negative net current $I_b=I_{ib}+I_{eb}$ crossing the external boundaries ($III$) at initial time steps is evident. Therefore $|\phi_\infty|$ increases (the charging cycle) to slow down fast electrons. The rate of increase slows (see Figure~\ref{fig:oneDtest} (b)) as fewer electrons can escape the growing potential barrier. This is evident since the resulting net current across the external boundaries is negligible from $2\mu s$ to $6\mu s$ (see Figure~\ref{fig:oneDtest} (c)). The minimum of the voltage curve is registered at around $6\mu s$, it represents the time at which ions begin to cross the external boundaries. $\phi_\infty$ begins to decrease (the discharging cycle) as fewer electron reflections are required to balance a now net positive current that peaks at $6.8\mu s$ (see Figure~\ref{fig:oneDtest}(c)). After this initial recovery, a further, but slower, decrease in $|\phi_\infty|$ occurs until the equilibrium state is achieved. After $24 \mu s$, the net current leaving the external boundaries fluctuates about zero and a steady-state value of $\phi_\infty=-31.59V$ is reached. The latter is similar to the theoretical initial value of $\phi_\infty^0=-32.20V$.

At the steady state, a zero net current $I_0=I_{i0}+I_{e0}$ is achieved across the thruster outlet boundary ($I$) as shown in Figure~\ref{fig:oneDtest}(d). This arises purely as a product of the self-consistent electric field coupling electrons to the ion beam, since the current-free condition is only enforced at the external boundaries; only quasi-neutrality is enforced at ($I$). After an initially net negative current, caused by the re-injection of electrons as per the circuit boundary condition, steady-state is achieved at around $5\mu s$. Lastly, Figure~\ref{fig:oneDtest}(e) provides the convergence of thrust which achieves steady-state at $24\mu s$, namely in the same time as $|\phi_\infty|$. The steady thrust is $F=401\mu N$.  

\subsubsection{\color{red}Virtual capacitance}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{Cind.eps}
    \caption{\color{red}Potential at infinity $\phi_\infty$ in function of the simulation time $t$ in the low-magnetisation case. Three values of the virtual capacitance $C$ are used: 0.8 nF (\textcolor{blue}\full); 0.4 nF (\textcolor{red}\full); and 0.2 nF (\full).}
    \label{fig:C_independance}
\end{figure}

{\color{red}In order to further investigate the stability of the new boundary conditions, the results obtained with different values of the virtual capacitance ($C$) have been compared in Figure~\ref{fig:C_independance} in terms of $\phi_\infty$. This analysis concerns the low-magnetisation ($B_0=100$ G) plume.} First, all three cases converge to the same steady state value of $\phi_\infty=34.56V$. Second, {\color{red}for smaller values of $C$}, the voltage drop in the charging cycle increases: around -60.8V, -63.5V and -66.1V for {\color{red}$C=0.8$, $0.4$ and $0.2$nF respectively.} Namely, lower values of $C$ cause a marginally increase in the ambipolar acceleration of the ions during the transient. Thus, the point at which ions begin to cross the external boundaries occurs $0.13\mu s$ and $0.22\mu s$ earlier for {\color{red}$C=0.8$ and $C=0.4$nF compared to $C=0.2$nF. Third, analogous to a simple capacitive circuit, the smaller the value of $C$ the higher the voltage drop but the smaller the discharging time.} This results in the equilibrium state being achieved at approximately the same simulation time ($15\mu s$) for all three cases. In conclusion, while the value of $C$ affects the plume during the transient phase, the solution at steady state is independent on $C$. This further confirms the robustness of the proposed simulation strategy.

{\color{red}It is important to note that smaller values of $C$ cause an increase of noise.} This is expected for a proportional-type control law (see Eq.~\ref{eqn:control}), since the value of $C$ places an effective resolution on the adjustment of $\phi_\infty$. It is therefore important to exercise care in the choice of the virtual capacitance. {\color{red}$C$ must be small enough} to create the voltage drop necessary to prevent the instability, but not so small as to introduce additional noise to the solution. For the remainder of the simulations in this work, {\color{red}$C=0.2$nF was chosen.}

%
%
%
\subsection{Domain independence}
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{domain_ind.eps}
    \caption{a) Electron density $n_e$ and b) plasma potential $\phi$ using the nominal $25R_0 \times 10R_0$, three-quarter $18.75R_0 \times 7.5R_0$ and half $12.5R_0 \times 5R_0$ domains. Dashed lines (\dashed) indicate the boundaries of the reduced domains.}
    \label{fig:domain_ind}
\end{figure}
%
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{axis_ind.eps}
    \caption{\color{red}a) Electron density along the $z$-axis; (b) plasma potential along the $z$ -axis; c) electron density along $z = 0,5R_0,10R_0$; and (d) plasma potential along $z = 0,5R_0,10R_0$. Domain sizes $25R_0\times10R_0$ (\full), $18.75R_0\times7.5R_0$ (\textcolor{red}{\opencircle}) and $12.5R_0\times5R_0$ (\textcolor{blue}{\opensquare}).}
    \label{fig:axis_ind}
\end{figure}
%
For the high-magnetisation case ($B_0=500$G), simulations are performed to demonstrate the domain independence of the results using domain sizes of $25R_0\times10R_0$ (nominal), $18.75R_0\times7.5R_0$ (three-quarter) and $12.5R_0\times5R_0$ (half). Both reduced domains converged to values of $\phi_\infty$ within $0.4V$ of the nominal $-37.75V$. A comparison of the steady-state electron density and plasma potential distributions across the domains is shown in Figure~\ref{fig:domain_ind}. The quantities have been averaged for 50000 time-steps after the flow has reached the steady-state ($N_p\sim8.4\times 10^5$). It can be seen that the shape of the plume obtained from both reduced domain simulations are in very good agreement with the nominal case. {\color{red}For a more quantitative analysis, the electron density and plasma potential are compared along the axis of symmetry ($r=0$). The same has been repeated along lines that span the domain radially at $z = 0$, $z=5R_0$ and $z=10R_0$.} This is shown in Figure~\ref{fig:axis_ind}. Along the axis, results agrees within 1\% for the electron density, and 3\% for the plasma potential (see Figure~\ref{fig:axis_ind}(a) and Figure~\ref{fig:axis_ind}(b) respectively). {\color{red}Along the radial lines, Figure~\ref{fig:axis_ind}(d) shows an agreement within 2\% in the plasma potential. Instead, the number density in the reduced domain simulations is up to 68\% higher toward the external boundaries for $r>5R_0$ compared to the nominal domain (see Figure~\ref{fig:axis_ind}(c)).} This difference may be attributed to the noise introduced due to the number of particles escaping and reflecting from the external boundary, which is no longer significantly removed from the thruster outlet. Nonetheless, the electron density within the core of the plume is in excellent agreement within 1\%. Overall, the comparisons demonstrate that the new set of boundary conditions provides a domain-independent solution within a tolerance smaller than the typical PIC noise. The same result holds true also for both the unmagnetised and low-magnetisation cases; figures have not been reported for the sake of brevity.
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{thrustDomain.eps}
    \caption{\color{red}Thrust $F$ in function of the axial truncation of the domain ($z/R_0$) for unmagnetised (\full), low-magnetisation (\textcolor{red}{\full}), and high-magnetisation (\textcolor{blue}{\full}) cases.}
    \label{fig:axial_thrust}
\end{figure}
%
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{thrustcontour.eps}
    \caption{\color{red}Thrust $F$ in function of the axial ($z/R_0$) and radial ($r/R_0$) truncations of the domain for the high-magnetisation case. The solid contour (\full) delimits plateau values and the dashed line (\dashed) represents the MN exit.}
    \label{fig:axial_contour}
\end{figure}
%

The final choice of domain size depends primarily on the phenomenon of interest. If only plume-spacecraft interactions are the desired result, significant computational savings can be realised by applying the new boundary conditions to a comparatively small domain. However, if the thrust is required, a domain of sufficient axial length is needed. {\color{red}Figure~\ref{fig:axial_thrust} shows the thrust $F(z)$ calculated for different axial truncations of the domain and for the three degrees of magnetisation. When the magnetic field is absent, the total axial flow momentum is conserved since no mechanism can exert force on the plasma; as a result $F(L_z)=F(0)=401\mu N$.} In the low-magnetization case, $F$ increases to a converged value of $830\mu N$ at $z\sim 12R_0$. With for high-magnetization, $F$ increases to reach a maximum of about $892\mu N$ at $z\sim 14R_0$ and then gradually decreases (by less than 3\%) to a plateaued value of $868\mu N$ at $z=20R_0$. The axial plane where the thrust establishes a plateau may be referred to as the exit of the MN. The axial domain length must therefore include this plane so as to yield the accurate value of thrust. It is clear therefore that the domain size required is proportional to the magnetic field strength. The radial domain width must also be large enough. Figure~\ref{fig:axial_contour} spatially maps the thrust $F(z,r)$ for both axial and radial truncations of the domain in the high-magnetisation case. {\color{red}The size of the domain required to obtain a plateau value of $F$ is given in Figure~\ref{fig:axial_contour} by the area bounded by the contour line. Accordingly, the domain must have an axial length $Z\gtrsim 20R_0$ and radial width $R\gtrsim 5.3R_0$ to predict properly the propulsive performance if $B_0=500$G.}

==> chap_3_SA.tex <==
\section{\color{red}Verification of the numerical methodology}

\begin{table*}[!htb]
\caption{\label{tab:verparams} \color{red} Simulation parameters.}
\lineup
\centering
\begin{indented}
\item[]\begin{tabular}{@{}llll@{}}
\br
Parameter                          &                               & Unscaled             & Scaled$^b$              \\ \mr
Thruster Outlet Radius               & $R_0$ [mm]                  & 7                   & -                    \\
Ion Mass (Xe)                      & $m_i$ [kg]                  & $2.18\times10^{-25}$ & $5.45\times10^{-23}$ \\
Propellent Mass Flow Rate          & $\dot{m}$ [mg/s]        & 0.15                & 2.37                \\
Reference Plasma Density           & $n_{*}$ [m$^{-3}$]              & $1.6\times10^{18}$     & -                    \\
Reference Neutral Density & $n_{g*}~[m^{-3}]$& $5.3\times 10^{19}$ & - \\
Reference Ion Temperature          & $T_{i*}$ [K]               & 298                  & -                    \\
Reference Electron Temperature     & $T_{e*}$ [eV]              & 5                    & -                    \\
Reference Neutral Temperature     & $T_{g*}$ [K] & 298 & - \\
Reference Bohm Speed              & $c_{*}$ [m/s]         & 1920                 & 30310                \\
Ion Current                        & $I_{i0}$ [A]                & 0.0755             & 1.19               \\
Electromagnet Radius                & $R_c$ [mm]                  & 25.2                   & -                    \\
Throat Magnetic Field Strength     & $B_0$ [G]                   & $0-1000$              & -                    \\ \mr
Axial Domain Length                & $L_z$ [m]                  & 0.250                  & -                    \\
Radial Domain Length               & $L_r$ [m]                  & 0.100                  & -                    \\
Simulated Time                     & $T$ $[\mu s]$                 & -                    & 80                   \\
Reference Debye Length             & $\lambda_{D*}$ [mm]        & 0.0186             & $0.500$              \\
Reference Plasma Frequency         & $\omega_{p*}$ [rad/s] & $8.02\times10^{10}$  & $2.98\times10^{8}$   \\
Electron Gyro-Frequency$^a$          & $\omega_{ce0}$ [rad/s]  & $1.10\times10^{10}$  & -                  \\
Number of Axial Cells              & $N_z$                         & -                    & 500                  \\
Number of Radial Cells             & $N_r$                         & -                    & 200                  \\ 
Number of Time-steps$^a$           & $N_t$                         & -                    & $1.58\times10^6$     \\
Steady-state Macro-particles               & $N_p$                         & -                    & $\approx 8\times10^5$    \\
\br
\end{tabular}
\item[] $^a$ $100G$.
\item[] $^b$ $f=250$, $\gamma=26.9$.
\end{indented}
\end{table*}

{\color{blue}This section demonstrates the robustness of the new boundary conditions. The verification is divided into two parts: First the steady-state stability is demonstrated against the classical open outflow boundary conditions \cite{b:levin2018, b:hu2017}. (i.e. constant electron current injected at the plasma source, absorption of all electrons reaching the open boundaries ($III$) and the zero-Neumann condition on the Poisson's equation).} {\color{red}Second, a domain independence study is presented, evaluating both macroscopic plasma parameters and the propulsive performance (i.e. thrust) with respect to both axial and radial domain dimensions.}

Table~\ref{tab:verparams} summarises the physical and numerical parameters which are used, unless otherwise specified, throughout this article. {\color{blue}Xenon is the propellant modelled, with the reference plasma properties assumed within the source typical of the operating conditions in a low-power (50W) HPT \cite{b:manente2019,b:magarotto2020,b:magarotto2020_3}. A purely divergent MN is produced by an electromagnet of radius $R_c$, positioned concentric with the thruster outlet of radius of $R_0$.} {\color{blue}Figure~\ref{fig:b_field}(a) illustrates the magnetic field topology $\mathbf{B}$ on the nominal simulation domain, normalised with its value at the magnetic throat, that is $B_0=|\mathbf{B}(0,0)|$. Before commencing the PIC simulations, the DSMC method was used to pre-compute the neutral gas density field given in Figure~\ref{fig:b_field}(b).} 
%
\begin{figure}[!b]
    \centering
    \includegraphics[width=\linewidth]{dsmcBfield.eps}
    \caption{\color{red}(a) Normalised magnetic field magnitude $|\mathbf{B}|/B_0$. The electromagnet has radius $R_c=3.6R_0$. (b) Neutral density $n_g$ from the DSMC simulation.}
    \label{fig:b_field}
\end{figure}
%

{\color{blue}The scaling factors applied to the ion/neutral mass and the vacuum permittivity are $f=250$ and $\gamma=26.9$ respectively. The latter value is chosen such that the thruster outlet ($I$) is resolved with 20 cells $R_0=20\tilde{\lambda}_{D*}$. The domain spans $L_z=25R_0$ in length and $L_r=10R_0$ in height, with a uniform mesh resolution of $\tilde{\lambda}_{D*}$. The time-step adopted satisfies $\Delta t \omega_{ce0}=0.35$ such that the electron gyro-motion is resolved in all the domain and the stability criterion on the resolution of the scaled plasma frequency \cite{b:birdsall2005} is also satisfied (see Table~\ref{tab:verparams}). The Poisson's equation is solved every $0.286\tilde{\omega}_{p*}/\omega_{ce0}$ iterations \cite{b:birdsall2005}. Neutrals are sub-cycled at a larger time-step according to their Courant–Friedrichs–Lewy (CFL) condition \cite{b:bird1998}.} Macro-particle weights are selected so as to maintain an average number per cell above 10 at the steady-state, {\color{red}as a result $N_p\approx8\times10^5$.} The steady-state is characterised by the number of macro-particles leaving the domain matching the number of newly injected macro-particles at the thruster outlet ($I$) within 0.01\% for a defined number of iterations.
%

%
%
%
\subsection{Steady-state stability}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{bctime.eps}
    \caption{Transient evolution of (a) Total number of macro-particles $N_p$ for ions (\fullcircle), electrons (\textcolor{red}{\full}) and neutrals (\textcolor{blue}{\full}) in the new model, and ions (\dashed) and electrons (\textcolor{red}{\dashed}) for open outflow conditions; (b) free-space potential $\phi_\infty$; (c) net current $I_0$ at the thruster outlet ($I$); (d) net current $I_b$ at the open boundaries ($III$); and (e) thrust $F$.}
    \label{fig:oneDtest}
\end{figure}
%
{\color{blue}The stability of the new model is assessed for the unmagnetised case (i.e. $B_0=0$), since results can be more easily compared to theoretical values}. The time-step is defined by $\Delta t \omega_{pe*}=0.05$. Figure~\ref{fig:oneDtest}(a) gives the evolution of the macro-particle count for both the new model and the open outflow conditions. Although both simulations start with a similar growth in ion count during the transient, the electron count peaks around $14\mu s$ with the open outflow boundary. Despite the number of ions continuing to increase, the electron count decreases, resulting in a growing charge imbalance. This eventually results in the formation of a virtual anode \cite{b:brieda2018,b:briedaThesis} around $32\mu s$, which is followed by gradual ion loss. The vast majority of electrons are lost, thus the simulation collapses; this is the 'numerical pump instability' \cite{b:brieda2018,b:briedaThesis}. No such instability is observed with the new model. The electron and ion populations closely trend each other. Steady-state is achieved near $34\mu s$, and the ion and electron counts remain invariant for the reminder of the simulation. There is negligible change in the neutral count.

To prove the new model can self-consistently calculate the potential drop across the plume $\phi_\infty$, Figure~\ref{fig:oneDtest}(b) plots its value against the simulation time. The trend mimics the voltage seen across the charging-discharging cycle of a capacitor \cite{b:griffiths2013}. Indeed, from Figure~\ref{fig:oneDtest}(c), an initially large negative net current $I_B=I_{iB}+I_{eB}$ at the open boundaries ($III$) is clear. Therefore $|\phi_\infty|$ increases (the charging cycle) to slow down fast electrons. The rate of increase slows (see Figure~\ref{fig:oneDtest} (b)) as fewer electrons can escape the growing potential barrier, and $I_B$ becomes negligible towards $10\mu s$ (see Figure~\ref{fig:oneDtest} (c)). The minimum of the voltage curve, at around $10\mu s$, represents the time at which ions begin to cross the open boundaries. $|\phi_\infty|$ begins to decrease (the discharging cycle) as fewer electron reflections are required to balance a now net positive current that peaks at $11\mu s$ (see Figure~\ref{fig:oneDtest}(c)). After this initial recovery, a further, but slower, decrease in $|\phi_\infty|$ occurs as the ion beam current- which is itself determined by the ambipolar acceleration of $|\phi_\infty|$- establishes an equilibrium state. After $39 \mu s$, $I_B$ fluctuates about zero and a steady-state value of $\phi_\infty=-30.7V$ is reached. This is similar to the theoretical initial value of $\phi_\infty^0=-32.2V$; it also falls between the values of $-28.9V$ and $-37.5V$ given by alternatives to Equation~\ref{eqn:phi0} in references \cite{b:lafleur2011} and \cite{b:merino2018kinetic} respectively.

At the steady-state, a zero net current $I_0=I_{i0}+I_{e0}$ is achieved across the thruster outlet boundary ($I$) as shown in Figure~\ref{fig:oneDtest}(d). This arises purely as a product of the self-consistent electric field coupling electrons to the ion beam, since the current-free condition is only enforced at the open boundaries; only quasi-neutrality is enforced at ($I$). After an initially net negative current, caused by the re-injection of electrons as per the circuit condition, steady-state is achieved at around $8\mu s$. Lastly, Figure~\ref{fig:oneDtest}(e) provides the convergence of thrust, which achieves steady-state in the same time as $\phi_\infty$ at $39\mu s$. The steady-state thrust is $F=431\mu N$.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{cind.eps}
    \caption{Evolution of the plasma potential at infinity $\phi_\infty$ for three values of the virtual free-space capacitance $C$: $0.2nF$ (\full); $0.4nF$ (\textcolor{red}\full); and $0.2nF$ (\textcolor{blue}\full).}
    \label{fig:C_independance}
\end{figure}

{\color{blue}The results obtained with different values of the virtual free-space capacitance $C$ have been compared in Figure~\ref{fig:C_independance} in terms of $\phi_\infty$. Firstly, all three cases converge to a similar steady-state value within an accuracy of $0.12V$. Second, {\color{red}for smaller values of $C$}, the voltage drop in the charging cycle increases: around $-62.8V$, $-65.5V$ and $-69.0V$ for {\color{red}$C=0.8$, $0.4$ and $0.2nF$ respectively.} This marginally increases the ambipolar acceleration of the ions during the transient. Thus, the point at which ions begin to cross the open boundaries ($III$) occurs $0.26\mu s$ and $0.22\mu s$ earlier for {\color{red}$C=0.2$ and $C=0.4$nF compared to $C=0.8$nF. Analogous to a simple capacitive circuit, an increase in the value of $C$ increases the rate of voltage drop, while also decreasing the discharging time and the voltage recovery. This results in the equilibrium state being achieved at approximately the same simulation time ($39\mu s$) for all three cases}.} To conclude, while the value of $C$ affects the plume during the transient phase, the solution at steady-state is independent of it. This further confirms the robustness of the proposed simulation strategy.

{\color{red}It is also important to note that smaller values of $C$ cause an increase in noise.} This is expected for a proportional-type control law (see Eq.~\ref{eqn:control}), since the value of $C$ places an effective resolution on the adjustment of $\phi_\infty$. It is therefore important to exercise care in the choice of virtual free-space capacitance. {\color{red}$C$ must be small enough} to create the voltage drop necessary to prevent the instability, but not so small as to introduce additional noise to the solution. For the remainder of the simulations in this work, {\color{red}$C=0.8nF$ was chosen.}{\color{blue} Indeed, values larger than this did not reliably suppress the instability.}

%
%
%
\subsection{Domain independence}
%
\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{domainind.eps}
    \caption{a) Electron density $n_e$ and b) plasma potential $\phi$ using the nominal $25R_0 \times 10R_0$, three-quarter $18.75R_0 \times 7.5R_0$ and half $12.5R_0 \times 5R_0$ domains. Dashed lines (\dashed) indicate the boundaries of the reduced domains.}
    \label{fig:domain_ind}
\end{figure*}
%
%
%\begin{figure}[!htb]
%    \centering
%    \includegraphics[width=\linewidth]{axis_ind.eps}
%    \caption{\color{red}a) Electron density along the $z$-axis; (b) plasma potential along the $z$ -axis; c) electron density along $z = 0,5R_0,10R_0$; and (d) plasma potential along $z = 0,5R_0,10R_0$. Domain sizes $25R_0\times10R_0$ (\full), $18.75R_0\times7.5R_0$ (\textcolor{red}{\opencircle}) and $12.5R_0\times5R_0$ (\textcolor{blue}{\opensquare}).}
%    \label{fig:axis_ind}
%\end{figure}
%
For the case of $B_0=600G$, simulations are performed to demonstrate the domain independence using domain sizes of $18.75R_0\times7.5R_0$ (three-quarter) and $12.5R_0\times5R_0$ (half) compared to the nominal $25R_0\times10R_0$. Both reduced domains converged to values of $\phi_\infty$ within $0.4V$ of the nominal $-37.8V$. A comparison of the steady-state electron density and plasma potential distributions across the domains is shown in Figures~\ref{fig:domain_ind}(a) and (b) respectively. It can be seen that the shape of the plume obtained from both reduced domain simulations are in very good agreement with the nominal case. {\color{red}For a more quantitative analysis, the electron density and plasma potential are compared along the axis of symmetry ($r=0$) in Figures~\ref{fig:domain_ind}(c) and (d). Along the axis, results agree within 4\% for the electron density, and 2\% for the plasma potential. {\color{blue}The largest disagreement occurs outside the periphery of the outermost magnetic field line connected to the source, approximated by the $10^{15}m^{-3}$ contour in Figure~\ref{fig:domain_ind}(a). The density in the reduced domain simulations is up to 68\% higher in this region compared to the nominal.} This difference may be attributed to the noise introduced due to the number of particles escaping and reflecting from the radial open boundary $(III)$, which is no longer significantly removed from the thruster outlet $(I)$. Nonetheless, the electron density within the core of the plume is in excellent agreement within 2\% on average. Overall, the comparisons demonstrate that the new set of boundary conditions provides a domain-independent solution within a tolerance smaller than the typical PIC noise.}
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{domainthrust.eps}
    \caption{\color{blue}a) Thrust $F$ for axial truncation of the domain for unmagnetised (\full), $100G$ (\textcolor{red}{\full}), and $600G$ (\textcolor{blue}{\full}) cases. b) Thrust $F$ for axial and radial truncation in the $600G$ case. The solid contour (\full) represents the value of final thrust; the dashed line (\dashed) represents the MN exit.}
    \label{fig:axial_thrust}
\end{figure}

%

The final choice of domain size depends primarily on the phenomenon of interest. If only plume-spacecraft interactions are desired, significant computational savings can be realised by applying the new boundary conditions to a comparatively small domain. However, if the thrust is required, a domain of sufficient axial length is needed. {\color{red}Figure~\ref{fig:axial_thrust}(a) shows the thrust $F(z)$ calculated for different axial truncation of the domain. When the magnetic field is absent, the total axial flow momentum is conserved since no mechanism can exert force on the plasma; as a result $F(L_z)=F(0)=431\mu N$.} In the $100G$ case, $F$ increases to a converged value of $643\mu N$ at $z\sim 13R_0$. For $600G$, $F$ tends to a value of $703\mu N$ at $z\sim18R_0$. This axial plane where the thrust establishes a plateau may be referred to as the exit of the MN, where plasma detachment occurs. The axial domain length must therefore include this plane so as to yield the accurate value of thrust. The domain size required therefore is proportional to the magnetic field strength.

The radial domain width must also be large enough. Figure~\ref{fig:axial_thrust}(b) spatially maps the thrust $F(z,r)$ for both axial and radial truncation of the domain in the $600G$ case. {\color{blue}The size of the domain required to obtain a plateau value of $F$ is given by the area bounded by the contour. Accordingly, the domain must have an axial length $L_z\gtrsim 18R_0$ and radial width $L_r\gtrsim 8R_0$ to not underestimate the propulsive performance for $B_0=600G$.}

\subsection{Experimental validation}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{expvalid.eps}
    \caption{\centering Experimentally measured data (\opencircle) with relative uncertainty bands and PIC output (\textcolor{red}{\full}) on the axis of the \textit{Piglet} reactor: a) Electron number density $n_e$, and b) Plasma potential $\phi$.}
    \label{fig:valid_plot}
\end{figure}

The results of the PIC are compared against the measurements performed in the \textit{Piglet} Helicon plasma reactor, filled with Argon gas at $0.04Pa$ as described in reference \cite{b:lafleur2011}. The case referred to as 'B' in \cite{b:lafleur2011} is the magnetic configuration considered, where a magneto-static field, generated only by the \textit{source coil}, provides a throat intensity of $B_0 = 4G$. The validation input parameters are given in Table \ref{tab:validparams}. The domain is a truncation of the physical vacuum chamber used in the experiment, such to allow the use of the open boundaries. The plasma source properties were taken directly from the experimentally measured values.

\begin{table*}[!htb]
\caption{\label{tab:validparams} Validation parameters}
\lineup
\centering
\begin{indented}
\item[]\begin{tabular}{llll}
\br
Parameter &                       & Unscaled             & Scaled$^a$               \\ \mr
Plasma Source Number Density                             & $n_0$ $[m^{-3}]$      & $5\times10^{16}$     & -                    \\
Ion Mass (Ar)                                            & $m_i$ $[kg]$          & $6.63\times10^{-26}$ & $1.66\times10^{-27}$ \\
Reference Ion Temperature                                & $T_{i^*}$ $[K]$       & 298                  & -                    \\
Reference Electron Temperature                           & $T_{e^*}$ $[eV]$      & 9                    & -                    \\
Ion Bohm Speed                                           & $c_{i^*}$ $[ms^{-1}]$ & 4650                 & 29400      \\ \mr
Axial Domain Length & $L_z$ $[m]$ & 0.25 & - \\
Radial Domain Length & $L_r$ $[m]$ & 0.13 & - \\\br       
\end{tabular}
\item[] $^a$ $f=40$, $\gamma=33.1$.
\end{indented}
\end{table*}

The results obtained for the electron density distribution and plasma potential, along the axis of the discharge, have been reported in Figure \ref{fig:valid_plot}(a) and Figure \ref{fig:valid_plot}(b). The experimental plasma potential has been normalised so as that $\phi_0=0$ at $z=0$. Due to the possible overestimation of the Langmuir probe sheath area by about 15\%, used to derive the measured number density in reference \cite{b:lafleur2011}, the errorbars are asymmetrical between -5\% and 27\%. 

Focusing on the axial density profile in Figure \ref{fig:valid_plot}(a), the experimental trend is reproduced by the PIC model; the maximum local error is 10\% at $z=0.05m$, well within the uncertainty bands reported. Concerning the plasma potential profile of Figure \ref{fig:valid_plot}(b), the PIC model again repeats the experimental trend within the quoted uncertainty in the RFEA measurements of $\pm$5\%. However, the PIC slightly overestimates the potential in the downstream region of the plume, up to $1.6V$ at the downstream boundary. Critically, the potential drop calculated by the PIC was $\phi_\infty=-37.7V$, in excellent agreement with the local plasma potential of $V_p=37.2V$ directly measured at the exit of the source tube in reference \cite{b:lafleur2011}. This, as well as the similarity in potential gradient observed at $z=0.25m$ in Figure \ref{fig:valid_plot}(b), confirms the reliability of the open boundary conditions in the new model.



==> chap_4_MM.tex <==
\section{Physical analysis}

In this section, the 2D spatial and 1D on-axis plasma profiles are first examined. Second, the effect of varying the MN field strength on the global parameters, including performance indicators, is presented. A more detailed discussion is given on the nature of electron thermodynamics in the MN, with particular focus on the role of collisions and the location of the detachment plane.

\subsection{Plasma Profiles}

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{spatialplots.eps}
    \caption{\centering Plasma spatial properties for the $B_0=600G$ case: a) electron number density $n_e$; b) plasma potential $\phi$; c) electron temperature $T_e$; d) ion axial velocity $u_i$.}
    \label{fig:spatial_plot}
\end{figure*}

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{profiles.eps}
    \caption{\centering Plasma on-axis profiles for $B_0=0$ (\full); $B_0=100G$ (\textcolor{red}{\dashed}); and $B_0=600G$ (\textcolor{blue}{\dashed}).}
    \label{fig:onaxis_plot}
\end{figure*}


Figure~\ref{fig:spatial_plot} shows the 2D spatial fields for the $B_0=600G$ case, including (a) the electron number density, (b) plasma potential, (c) electron temperature and (d) ion axial velocity. The plasma follows the magnetic field lines of the MN, low divergence of the plume and a small electron void near the outer region of the thruster exit in Figure~\ref{fig:spatial_plot}(a).

A notable feature is observed in the potential field of Figure~\ref{fig:spatial_plot}(b): a radially non-monotonic dependence. This is characterised by an effective potential well near the vacuum interface line (the outermost magnetic field line starting at edge of plasma source boundary). This has been noted in a number of magnetically confined plasmas \cite{b:collard2019,b:chen2020} and can be interpreted as the consequence of charge separation that results from ions with sufficient radial energy surpassing the attached electrons, causing secondary ion expansion beyond the vacuum interface line in Figure. The potential well forms to counter this radial ion inertia and return the ion streamlines back toward the field-aligned electron trajectories. This is clearly seen in Figure~\ref{fig:spatial_plot}(d) by the discontinuity in ion axial velocity along the vacuum interface line, particularly at large $r$ for the $4000ms^{-1}$ contour. 

Cooling of electrons downstream in Figure \ref{fig:spatial_plot}(c) occurs as electron thermal energy is evidently converted to ion kinetic energy, facilitated by the ambipolar potential drop, with the magnetic field acting as a mediating factor. Note the regions of high $T_e>6eV$ at the radial peripheries of the thruster exit, beyond the vacuum interface line, occur since only the most highly-energetic electrons can detach from the MN in this region.

In order to provide a more quantitative comparison on the effect of the MN field strength, 1D plasma profiles have been sampled along the z-axis in Figure~\ref{fig:onaxis_plot} for $B_0=0,~100$ and $600G$. From Figure~\ref{fig:onaxis_plot}(a), the increased radial confinement of the plume from the application of the MN yields much higher plasma density downstream, but there is no significant change between $100G$ and $600G$. The MN effect tends to increase electron current due to the $\mathbf{v}_e\times \mathbf{B}$ force exerted on electrons. As a consequence, the potential drop increases with $B_0$ (Figure \ref{fig:onaxis_plot}(b)) so as to maintain the current-free plume. Consistently, the ion axial speed increases with $B_0$ (Figure \ref{fig:onaxis_plot}(c)). The on-axis velocity of ions in the presence of the MN is observed to be smaller than that in the absence of MN until $z\sim3R_0$ and the crossing point on the ion velocity profile is consistent with the result on the potential profile. It is interesting to note that the potential drop/acceleration occurs in a larger axial span in the magnetised cases; indeed, for both MN strengths, the potential drop of the near plume $z<5R_0$ is smaller, while the potential drop in the far plume is much larger and continuing to drop at a faster rate. This might be explained with mass conservation, since the ion beam divergence for the unmagnetised case is much higher, so a faster expansion is expected.

The electron cooling is reduced with increase in $B_0$ (Figure \ref{fig:onaxis_plot}(d)). It is reasonable to associate the slower cooling of the electrons to the increased plume confinement and so a reduced loss of energy through the periphery of the MN; this enables more electron energy to be available downstream. Strong temperature
anisotropy is developed as shown in Figures \ref{fig:onaxis_plot}(e) and (f). $T_{ex}$ decays to a non-zero value ($\sim 4eV$ for both MN strengths), while $T_{er}$ decays to near-zero. Interestingly,
a weaker MN means more free electrons, and this marginally increases $T_{ex}$ and decreases greatly $T_{er}$, resulting in more anisotropy and a smaller mean temperature seen in Figure \ref{fig:onaxis_plot}(d). Indeed, this anisotropy confirms the electrothermal conversion of electron internal energy into ion axial kinetic energy within the MN.

\subsection{Global Parameters}

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{perform.eps}
    \caption{\centering Effect of MN field strength on a) Thrust $F$; b) potential drop $|\phi_\infty|$ and c) Ion divergence angle $\bar{\theta}_{i}$}
    \label{fig:param}
\end{figure*}

The performance of the MNs is illustrated in Figure \ref{fig:param}. As the magnetic field strength increases, thrust also increases at a diminishing rate. The magnetic thrust in the $100G$ case accounts for approximately 50\% of the total thrust, but increasing the MN up to $1200G$ plateaus at a magnetic thrust of around 65\%, showing there is limit to the performance enhancement the MN can provide. The gain in thrust performance between the unmagnetised and magnetised cases is namely due to the increased radial confinement of ions and the corrsponding increase in downstream density; indeed there is a clear trend in the thrust of Figure \ref{fig:param}(a) and plume divergence $\bar{\theta}_i=\langle cos^{-1}(\mathbf{v}_i\cdot\mathbf{1}_z/|\mathbf{v}_i|) \rangle_i$ of Figure \ref{fig:param}(c). As $B_0$ is further increased, the additional thrust is due to the higher ion axial velocity achieved in association with the greater potential drop, seen in Figure \ref{fig:param}(b). The potential barrier must increase to balance an increasing number of free electrons induced by the MN field strength. Note, that in practice, the MN effect on performance is far more complex because it also affects the source region (not modelled in this work). The magnetic field strength affects the source confinement \cite{b:magarotto2020}, deposition of power into the plasma \cite{b:takahashi2019}, and the electron distribution function \cite{b:lafleur2015} of the discharge into the MN throat.

\subsection{Electron thermodynamics}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{gammafit.eps}
    \caption{\centering Polytropic coefficient fitting of the $600G$ case.}
    \label{fig:gamma_fit}
\end{figure}

The electron cooling in MN exspansions may be described, locally and globally, by a polytropic relation $(T_e/T_{e0}=(n_e/n_{e0})^{\gamma_e-1}$ where $\gamma_e$ is the polytropic coefficient. This is given by the best linear fitting of

\begin{equation}
    \gamma_e \sim 1+\frac{n_e}{T_e}\frac{dn_e}{dT_e}
\end{equation}

and is calculated by the regression of the $log_{10}T_e$ versus $log_{10}n_e$ relation, an example of which is given in Figure \ref{fig:gamma_fit} for the $600G$ case. The average value is shown to be $\bar{\gamma}_e\sim1.16$, but it is clear that a single polytropic coefficient cannot represent the electron cooling in the MN. Three separate regions are therefore identified for a piecewise polytropic relationship: 1) For most of the expansion in Figure \ref{fig:gamma_fit}, there is a region with $\gamma_{eM}\sim1.13$. 2) Far downstream there exists a region with a markedly greater value $\gamma_{eD}\sim1.30$. 3) The region nearest the MN throat does not quite conform to the fitting of $\gamma_{eM}$, but instead has a value $\gamma_{eT}\sim1.21$ (the fitting is not shown on Figure \ref{fig:gamma_fit} for clarity). 

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{gammas.eps}
    \caption{\centering The values of the polytropic coefficients, inferred using the linear regression, as a function of $B_0$.}
    \label{fig:gamma_b0}
\end{figure}

For all cases, the break between the first and second polytropic regions agree with the locations of the MN detachment planes identified in Figure \ref{fig:axial_thrust}. It can therefore be inferred that the first region is where the electrons are well-magnetised and frozen to the magnetic field lines, but the second region represents that where the plasma has detached from the MN and so the electron cooling is the same as that for an unmagnetised expansion. The third region possesses a value that lies between the coefficients found in the first two regions, therefore it may be assumed that the electron fluid in this region is not fully attached to the MN.

Figure \ref{fig:gamma_b0} shows the effect of the MN strength on the coefficients describing the different polytropic regions. Notably, the value of $\gamma_{eD}$ is approximately constant- and equal to the unmagnetised average $\bar{\gamma}_e$- for all cases. This confirms this region is post plasma detachment. Increasing the magnetic field strength reduces the average electron cooling rate, tending to $\bar{\gamma}\sim 1.16$ for $600-1200G$. This is in good agreement with experimentally measured $\bar{\gamma}_e$ for MN plasmas, which is reported to vary between 1.1 and 1.23 \cite{b:collard2019,b:correyero2019}, with measurements of $\bar{\gamma}_e$ = 1.15 $\pm$ 0.02 reported also in reference \cite{b:little2016}. A theoretical limit of $\bar{\gamma}_e$ = 1.16 was also reported in reference \cite{b:littlephd}. 

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{hall.eps}
    \caption{\centering a) Electron Hall parameter $\Omega_e$ along the axis for the $100G$ (\textcolor{red}{\full}) and $600G$ (\textcolor{blue}{\full})}. b) Local polytropic coefficient $\gamma_e$ along the axis for the unmagnetised case (\full), $100G$ (\textcolor{red}{\full}) and $600G$ (\textcolor{blue}{\full}).
    \label{fig:hall}
\end{figure*}

Sufficiently upstream near the thtuster exit, electron-neutral/ion collisions act to de-magnetise the electrons.  The plasma remains dominated by collisions in the near-field plume. This precludes the
accelerating action of the magnetic field until the neutral gas
becomes sufficiently sparse that the electrons become
magnetised. To evaluate this mechanism, consider the
total electron Hall parameter

\begin{equation}
    \Omega_e = \frac{e|\mathbf{B}|}{m_e\nu}
\end{equation}

where $\nu$ is the total of the electron-neutral and electron-ion collision frequencies calculated from the MCC module of the simulations. Physically, if the Hall parameter is large, an electron undergoes many gyrorotations between collisions. Conversely, if the Hall parameter is small, an electron undergoes either partial or few gyrorotations between collisions. During each collision with a neutral an electron can move to an adjacent MN streamline; a large collision frequency results in enhanced cross-field electron transport. In Figure \ref{fig:hall}(a) a comparison of the total electron Hall parameter between the $100G$ and $600G$ is shown. The detachment planes of these MN strengths were previously identified as $13R_0$ and $18R_0$, where $\Omega_e$ takes values of 100 and 550 respectively—values that are indicative of a magnetised electron fluid. Fundamentally, comparison to the local polytropic coefficient of Figure \ref{fig:hall}(b) show a positive trend to the between Hall parameter; as the MN field strength increases the Hall parameter increases within the near-field while the polytropic coefficient in the throat region increases. Physically, this trend states that as the magnetic field increases the electrons in the near-field plume are becoming more magnetised closer to the thruster exit, yet the electrons tend to the unmagnetised cooling behaviour. The fact that the plasma detachment occurs at the aforementioned values of $\Omega_e$, suggests that the electrons are also at least partially detached at $z<R_0$ and $z<0.4R_0$ for $100G$ and $600G$ respectively. 











==> chap_5_SA.tex <==
\section{Physical analysis}

In this section, the 2D spatial and 1D on-axis plasma profiles are first examined. Second, the effect of varying the MN field strength on the global parameters, including performance indicators, is presented. A more detailed discussion is given on the nature of electron thermodynamics in the MN, with particular focus on the role of collisions.

\subsection{Plasma Profiles}

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{spatialplots.eps}
    \caption{\centering Plasma spatial properties for the $B_0=600G$ case: a) electron number density $n_e$; b) plasma potential $\phi$; c) electron temperature $T_e$; d) ion axial velocity $u_i$.}
    \label{fig:spatial_plot}
\end{figure*}

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{profiles.eps}
    \caption{\centering Plasma on-axis profiles for $B_0=0$ (\full); $B_0=100G$ (\textcolor{red}{\dashed}); and $B_0=600G$ (\textcolor{blue}{\dashed}).}
    \label{fig:onaxis_plot}
\end{figure*}


Figure~\ref{fig:spatial_plot} shows the 2D spatial fields for the $B_0=600G$ case, including (a) the electron number density, (b) plasma potential, (c) electron temperature and (d) ion axial velocity. The plasma follows the magnetic field lines of the MN, with low divergence of the plume and a small electron void near the outer region of the thruster exit in Figure~\ref{fig:spatial_plot}(a). The plasma properties propagate monotonically downstream under the dominance of a self-consistently developed ambipolar electric field.

A notable feature is observed in the potential field of Figure~\ref{fig:spatial_plot}(b): a radially non-monotonic dependence. This is characterised by an effective potential well near the vacuum interface line (the outermost magnetic field line starting at edge of thruster exit boundary). This has been noted in a number of magnetically confined plasmas \cite{b:collard2019,b:chen2020} and can be interpreted as the consequence of charge separation that results from ions with sufficient radial energy surpassing the attached electron fluid, causing secondary ion expansion beyond the vacuum interface line. The potential well forms to counter this radial ion inertia and return the ion streamlines back toward the MN-aligned electron trajectories. This is clearly seen in Figure~\ref{fig:spatial_plot}(d) by the discontinuity in ion axial velocity along the vacuum interface line, particularly at large $r$ for the $4000ms^{-1}$ contour. 

{\color{blue}It should be noted that the potential peak magnitude near the thruster exit is much larger than that observed in the PIC simulations of reference \cite{b:chen2020}. This may be explained by the inclusion of CEX collisions in this work. Radially accelerating CEX ions enhance the secondary ion expansion, increasing the positive space charge and hence the strength of the potential barrier. The difference in ion mass ($m_i/m_e=1836$ in \cite{b:chen2020}) might also explain the difference since, in theory, heavier ions should require a larger electric field to return their trajectories into the MN. }

Cooling of electrons downstream in Figure \ref{fig:spatial_plot}(c) occurs as electron thermal energy is evidently converted to ion kinetic energy, facilitated by the ambipolar potential drop, with the magnetic field acting as a mediating factor. Note the regions of high $T_e>6eV$ at the radial peripheries of the thruster exit, beyond the vacuum interface line, occur since only the most highly-energetic electrons can detach from the MN in this region.

In order to provide a more quantitative comparison on the effect of the MN field strength, 1D plasma profiles have been sampled along the z-axis in Figure~\ref{fig:onaxis_plot} for $B_0=0,~100$ and $600G$. From Figure~\ref{fig:onaxis_plot}(a), the increased radial confinement of the plume from the application of the MN yields much higher plasma density downstream, but there is no significant change between $100G$ and $600G$. The MN effect tends to increase electron current due to the $\mathbf{v}_e\times \mathbf{B}$ force exerted on electrons. As a consequence, the potential drop increases with $B_0$ (Figure \ref{fig:onaxis_plot}(b)) so as to maintain the current-free plume. Consistently, the ion axial speed increases with $B_0$ (Figure \ref{fig:onaxis_plot}(c)). The on-axis velocity of ions in the presence of the MN is observed to be smaller than that in the absence of MN until $z\sim3R_0$ and the crossing point on the ion velocity profile is consistent with the result on the potential profile. It is interesting to note that the potential drop/acceleration occurs in a larger axial span in the magnetised cases; indeed, for both MN strengths, the potential drop of the near plume $z<5R_0$ is smaller, while the potential drop in the far plume is much larger and continuing to drop at a faster rate. This might be explained with mass conservation, since the ion beam divergence for the unmagnetised case is much higher, so a faster expansion is expected.

The electron cooling is reduced with increase in $B_0$ (Figure \ref{fig:onaxis_plot}(d)). It is reasonable to associate the slower cooling of the electrons to the increased plume confinement and so a reduced loss of energy through the periphery of the MN; this enables more electron energy to be available downstream. Strong temperature
anisotropy is developed as shown in Figures \ref{fig:onaxis_plot}(e) and (f). $T_{ex}$ decays to a non-zero value ($\sim 4eV$ for both MN strengths), while $T_{er}$ decays to near-zero. Interestingly,
a weaker MN means more free electrons, and this marginally increases $T_{ex}$ and decreases greatly $T_{er}$, resulting in more anisotropy and a smaller mean temperature seen in Figure \ref{fig:onaxis_plot}(d). Indeed, this anisotropy confirms the electrothermal conversion of electron internal energy into ion axial kinetic energy within the MN.

\subsection{Global Parameters}

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{perform.eps}
    \caption{\centering Effect of MN field strength on a) Thrust $F$; b) potential drop $|\phi_\infty|$ and c) Ion divergence angle $\bar{\theta}_{i}$}
    \label{fig:param}
\end{figure*}

The performance of the MNs is illustrated in Figure \ref{fig:param}. As the magnetic field strength increases, thrust also increases at a diminishing rate. The magnetic thrust in the $100G$ case accounts for approximately 50\% of the total thrust, but increasing the MN up to $1200G$ plateaus at a magnetic thrust of around 65\%, showing there is limit to the performance enhancement the MN can provide. The gain in thrust performance between the unmagnetised and magnetised cases is namely due to the increased radial confinement of ions and the corrsponding increase in downstream density; indeed there is a clear trend in the thrust of Figure \ref{fig:param}(a) and plume divergence $\bar{\theta}_i=\langle cos^{-1}(\mathbf{v}_i\cdot\mathbf{1}_z/|\mathbf{v}_i|) \rangle_i$ of Figure \ref{fig:param}(c). As $B_0$ is further increased, the additional thrust is due to the higher ion axial velocity achieved in association with the greater potential drop, seen in Figure \ref{fig:param}(b). The potential barrier must increase to balance an increasing number of free electrons induced by the MN field strength. Note, that in practice, the MN effect on performance is far more complex because it also affects the source region (not modelled in this work). The magnetic field strength affects the source confinement \cite{b:magarotto2020}, deposition of power into the plasma \cite{b:takahashi2019}, and the electron distribution function \cite{b:lafleur2015} of the discharge into the MN throat.

\subsection{Electron thermodynamics}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{gammafit.eps}
    \caption{\centering Polytropic coefficient fitting of the $600G$ case.}
    \label{fig:gamma_fit}
\end{figure}

The electron cooling in MN expansions may be described, locally and globally, by a polytropic relation $(T_e/T_{e0}=(n_e/n_{e0})^{\gamma_e-1}$ where $\gamma_e$ is the polytropic coefficient. This is given by the best linear fitting of

\begin{equation}
    \gamma_e \sim 1+\frac{n_e}{T_e}\frac{dn_e}{dT_e}
\end{equation}

and is calculated by the regression of the $log_{10}T_e$ versus $log_{10}n_e$ relation, an example of which is given in Figure \ref{fig:gamma_fit} for the $600G$ case. The average value is shown to be $\bar{\gamma}_e\sim1.16$, but it is clear that a single polytropic coefficient cannot represent the electron cooling in the MN. Three separate regions are therefore identified for a piecewise polytropic relationship: {\color{blue} Nearest the thruster exit is a region with a mildly-adiabatic value $\gamma_{eT}\sim1.21$. Further downstream, and for most of the expansion, there is a region with near-isothermal $\gamma_{eM}\sim1.13$. Finally, farther downstream, there exists a region with a markedly greater value $\gamma_{eD}\sim1.30$. }

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{gammas.eps}
    \caption{\centering The values of the polytropic coefficients, inferred using the linear regression, as a function of $B_0$.}
    \label{fig:gamma_b0}
\end{figure}

For all cases, the break between the second and third polytropic regions agree with the locations of the MN detachment planes identified in Figure \ref{fig:axial_thrust}. It can therefore be inferred that the second region is where the electrons are well-magnetised and frozen to the magnetic field lines, but the third region represents that where the plasma has detached from the MN and so the electron cooling is the same as that for an unmagnetised expansion. The first region possesses a value that lies between the coefficients found in the first two regions, therefore it may be assumed that the electron fluid in this region is not fully attached to the MN.

Figure \ref{fig:gamma_b0} shows the effect of the MN strength on the coefficients describing the different polytropic regions. Notably, the value of $\gamma_{eD}$ is approximately constant- and equal to the unmagnetised average $\bar{\gamma}_e$- for all cases. This confirms this region is post plasma detachment. Increasing the magnetic field strength reduces the average electron cooling rate, tending to $\bar{\gamma}\sim 1.16$ for $600-1200G$. This is in good agreement with experimentally measured $\bar{\gamma}_e$ for MN plasmas, which is reported to vary between 1.1 and 1.23 \cite{b:collard2019,b:correyero2019}, with measurements of $\bar{\gamma}_e$ = 1.15 $\pm$ 0.02 reported also in reference \cite{b:little2016}. A theoretical limit of $\bar{\gamma}_e$ = 1.16 was also reported in reference \cite{b:littlephd}. 

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{hall.eps}
    \caption{\centering a) Electron Hall parameter $\Omega_e$ along the axis for the $100G$ (\textcolor{red}{\full}) and $600G$ (\textcolor{blue}{\full})}. b) Local polytropic coefficient $\gamma_e$ along the axis for the unmagnetised case (\full), $100G$ (\textcolor{red}{\full}) and $600G$ (\textcolor{blue}{\full}).
    \label{fig:hall}
\end{figure*}

{\color{blue}Consider the total electron Hall parameter

\begin{equation}
    \Omega_e = \frac{e|\mathbf{B}|}{m_e\nu}
\end{equation}

where $\nu=\nu_{en}+\nu_{ei}$ is the total of the electron-neutral and electron-ion collision frequencies calculated from the MCC module of the simulations}. During each collision with a neutral or ion, an electron can move to an adjacent MN streamline; a large collision frequency results in enhanced cross-field electron transport. In Figure \ref{fig:hall}(a) a comparison of the total electron Hall parameter between the $100G$ and $600G$ is shown. The detachment planes of these MN strengths were previously identified as $13R_0$ and $18R_0$, where $\Omega_e$ takes values of 17 and 90 respectively—values that are indicative of a fairly weakly-magnetised electron fluid. Fundamentally, comparison to the polytropic fitting of Figure \ref{fig:gamma_b0} shows a trend to the Hall parameter; as the MN field strength increases the Hall parameter increases within the near-field while the polytropic coefficient in the throat region increases. The fact that the plasma detachment occurs at the aforementioned values of $\Omega_e$, suggests that the electrons are also at least partially detached at $z<R_0$ and $z<0.4R_0$ for $100G$ and $600G$ respectively.  

This shows that, sufficiently upstream near the thruster exit, electron-neutral/ion collisions act to de-magnetise the electrons.  The plasma remains dominated by collisions in the near-field plume. This collisionality reduces the plasma conduction and thermalises the electron distribution, increasing the near-throat polytropic index towards the adiabatic. This precludes the accelerating action of the magnetic field until the neutral gas becomes sufficiently sparse ($|dn_g/dz|>|d|\mathbf{B}|/dz|$ in this case) that the electrons become strongly magnetised again. Increasing $B_0$ reduces the collisional transport of electrons near the throat, which decreases $\gamma_{eT}$ closer to the isothermal.

{\color{blue}A high neutral density near the thruster exit also leads to CEX ion collisions, which acts as a drag term on the ion fluid. To assess this, the CEX mean free path $\lambda_{CEX}$ can be compared to the characteristic length scale of ambipolar acceleration $(-E_z/|\phi|)^{-1}$. $\lambda_{CEX}$ can be estimated from the PIC simulation as $\lambda_{CEX} \sim |\mathbf{v}_i|/\nu_{CEX}$, where $\nu_{CEX}$ is the CEX collsion frequency taken from the MCC module. If the CEX mean free path is shorter than the acceleration length scale the ions are experiencing a drag force through frequent CEX collisions. Otherwise, the ion acceleration is not significantly
impeded by these collisions. The on axis length scales are given in Figure \ref{fig:hall}(b). The axial location at which
the CEX mean free path becomes equal to the acceleration
length scale appears independent of the MN field strength at $z/R_0=1.6$. The action of this CEX drag may explain why the potential drop, and subsequent ion velocity, in the near exit region is identical in each case presented in Figure \ref{fig:onaxis_plot}. This behaviour is unlikely to hold true if the plasma source was included in the model; the effect of the MN field strength would alter the ionisation ratio and neutral density, potentially leading to a mismatch between the MN throat and ion Bohm speed.} 









